On Delay-Optimal Scheduling in Queueing Systems with Replications

In modern computer systems, jobs are divided into short tasks and executed in parallel. Empirical observations in practical systems suggest that the task service times are highly random and the job service time is bottlenecked by the slowest straggling task. One common solution for straggler mitigation is to replicate a task on multiple servers and wait for one replica of the task to finish early. The delay performance of replications depends heavily on the scheduling decisions of when to replicate, which servers to replicate on, and which job to serve first. So far, little is understood on how to optimize these scheduling decisions for minimizing the delay to complete the jobs. In this paper, we present a comprehensive study on delay-optimal scheduling of replications in both centralized and distributed multi-server systems. Low-complexity scheduling policies are designed and are proven to be delay-optimal or near delay-optimal in stochastic ordering among all causal and non-preemptive policies. These theoretical results are established for general system settings and delay metrics that allow for arbitrary arrival processes, arbitrary job sizes, arbitrary due times, and heterogeneous servers with data locality constraints. Novel sample-path tools are developed to prove these results.

==> appendices.tex <==
% !TEX root = ./replication.tex
\ifreport
\appendices
\else
\appendix
\fi
\section{Proofs of Lemmas~1-3 and Corollaries 1-2} \label{app0}
\ifreport
\begin{proof}[Proof of Lemma \ref{lem1}]
\else
\begin{proof}[of Lemma \ref{lem1}]
\fi
First, fix the sequence of task completion times as $\bm{T}(\pi)=\bm{t}$ for all $\pi\in\Pi$. Because a job is completed at the time that the last task of the job is completed, each job completion time $C_i(\pi)$ must be equal to one element of $\bm{t}$. Using condition 2 and the sample-path optimality of the preemptive SRPT discipline \cite{Schrage68,Smith78}, one can obtain that for all $\pi\in\Pi$ and $\bm{t}\geq\bm{0}$
\begin{align}
[\bm{C}_{\uparrow} (P')|\bm{T}(P')=\bm{t}] \leq[\bm{C}_{\uparrow} (\pi)|\bm{T}(\pi)=\bm{t}],\nonumber
\end{align} 
where $\bm{C}_{\uparrow} (\pi)= (C_{(1)}(\pi),\ldots,$ $C_{(n)}(\pi))$ is the increasing time sequence of job completions. In addition, using the proof arguments in \cite{Schrage68,Smith78}, we can show that $[\bm{C}_{\uparrow} (P') | \bm{T}(P')=\bm{t}]$ is an increasing function of $\bm{t}$. This implies
\begin{align}\label{eq_order}
[\bm{C}_{\uparrow} (P')|\bm{T}(P')=\bm{t}] \leq[\bm{C}_{\uparrow} (\pi)|\bm{T}(\pi)=\bm{t}'],
\end{align} 
whenever $\bm{0}\leq\bm{t}\leq \bm{t}'$. On the other hand, condition 1 tells us that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}\label{eq_order_}
[\bm{T}(P')|\mathcal{I}] \leq_{\text{st}}[\bm{T}(\pi)|\mathcal{I}].
\end{align} 
%Therefore, 
%\begin{align}
%[{D}_{\text{avg}}(\bm{C}_{} (P))|\mathcal{I}] \leq_{\text{st}}[{D}_{\text{avg}}(\bm{C}_{} (\pi))|\mathcal{I}].\nonumber
%\end{align} 
According to Theorem 6.B.3 and Theorem 6.B.16(c) of \cite{StochasticOrderBook}, we can obtain from  \eqref{eq_order} and \eqref{eq_order_} that
\begin{align}\label{eq_order_1}
[\bm{C}_{\uparrow} (P')|\mathcal{I}] \leq_{\text{st}}[\bm{C}_{\uparrow} (\pi)|\mathcal{I}].
\end{align} 
Combining this and condition 3, we can get
\begin{align}
[\bm{U}_{\uparrow} (P)|\mathcal{I}] \leq_{\text{st}}[\bm{C}_{\uparrow} (\pi)|\mathcal{I}].\nonumber
\end{align} 
Since ${D}_{\text{avg}}\in \mathcal{D}_{\text{sym}}$ is symmetric and increasing, we can obtain that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}
&[{D}_{\text{avg}}(\bm{U} (P))|\mathcal{I}]=[{D}_{\text{avg}}(\bm{U}_{\uparrow} (P))|\mathcal{I}] \nonumber\\
\leq_{\text{st}}&[{D}_{\text{avg}}(\bm{C}_{\uparrow} (\pi))|\mathcal{I}] = [{D}_{\text{avg}}(\bm{C} (\pi))|\mathcal{I}],\nonumber
\end{align} 
where the inequality follows from Theorem 6.B.16(a) of \cite{StochasticOrderBook}. By this, \eqref{eq_lem1_1} is proven.

If condition 3 is replaced by $P'=P$, then \eqref{eq_lem1_2} follows from \eqref{eq_order_1} and Theorem 6.B.16(a) of \cite{StochasticOrderBook}. This completes the proof.
%In addition, 
%
%Let $[{D}_{\text{avg},\pi} |\mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,$ $\ldots, t_J)]$ denote the average delay of policy $\pi$ for given parameters $\mathcal{I}$ and task completion instants $(t_1,\ldots, t_J)$. According to the sample-path optimality of the preemptive SRPT discipline \cite{Schrage68,Smith78}, $[{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots,$ $ t_J)]$ is minimized among all policies in $\Pi$, if each completed task belongs to a job with the fewest remaining tasks. By condition 2, policy $P$ satisfies this requirement, and hence
%\begin{align}
%&~~~[{D}_{\text{avg},P} | \mathcal{I}, (t_{1,P},\ldots,t_{J,P}) = (t_1,\ldots, t_J)] \nonumber\\
%&\leq [{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)],~\forall~\pi\in\Pi.\nonumber
%\end{align}
%Further, $[{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)]$ is an increasing function of $(t_1,\ldots, t_J)$, because if task completions are postponed, the job completions are also postponed.
%Therefore, for any $\pi\in\Pi$, we have
%\begin{align}\label{eq_order}
%&~~~[{D}_{\text{avg},P} | \mathcal{I}, (t_{1,P},\ldots,t_{J,P}) = (t_1,\ldots, t_J)] \nonumber\\
%&\leq [{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1',\ldots,t_J')],\nonumber\\
%&~~~~~~~~~~~~~~~~~~~~\text{whenever}~(t_1,\ldots, t_J)\leq (t_1',\ldots,t_J').
%\end{align}
%By condition 1, we can obtain 
%\begin{align}\label{eq_order_}
%(t_{1,P},\ldots,t_{J,P})\leq_{\text{st}}(t_{1,\pi},\ldots,t_{J,\pi}),~\forall~\pi\in\Pi.
%\end{align}
%With \eqref{eq_order} and \eqref{eq_order_}, we can use the standard construction argument
% in Theorem 6.B.3 of \cite{StochasticOrderBook} to show that for all $\pi\in\Pi$
%\begin{align}\label{eq_order1}
%\!\!\!\![{D}_{\text{avg},P}, (t_{1,P},\ldots,t_{J,P})| \mathcal{I}] \leq_{\text{st}} [{D}_{\text{avg},\pi}, (t_{1,\pi},\ldots,t_{J,\pi}) | \mathcal{I}].\!\!\!\!
%\end{align}
%Then, \eqref{eq_thm1} follows from \eqref{eq_order1} and Theorem 6.B.16 (c) of \cite{StochasticOrderBook}. 
%Finally, \eqref{eq_thm1_1} follows from condition 3, \eqref{eq_thm1}, and Eq (6.B.4) of \cite{StochasticOrderBook}.
%By Theorem \ref{thm1}, for all $\mathcal{I}$, we have
%\begin{align}
%\mathbb{E}[{D}_{\text{avg},P'}| \mathcal{I}]  \leq \mathbb{E}[{D}_{\text{avg},\pi}| \mathcal{I}],~\forall~\pi\in\Pi.\nonumber
%\end{align}
%%Hence,
%%\begin{align}
%%[{D}_{\text{avg},P'}| \mathcal{I}]  \leq_{\text{st}} [{D}_{\text{avg},\pi}| \mathcal{I}],~\forall~\pi\in\Pi.\nonumber
%%\end{align}
%%
%%Because $G$ is independent of $P$, $P'$, and $\mathcal{I}$, by Theorem 1.A.3 (b) of \cite{StochasticOrderBook}, we have
%%\begin{align}
%%[{D}_{\text{avg},P'}| \mathcal{I}] +G  \leq_{\text{st}} [{D}_{\text{avg},\pi}| \mathcal{I}] + G,~\forall~\pi\in\Pi.\nonumber
%%\end{align}
%This, together with condition 3, implies %\eqref{eq_thm2}. Finally, 
%\eqref{eq_thm2_1}. % follows from \eqref{eq_thm2} and Eq (6.B.4) of \cite{StochasticOrderBook}.
\end{proof}
\ifreport
\begin{proof}[Proof of Corollary \ref{coro1}]
\else
\begin{proof}[of Corollary \ref{coro1}]
\fi
Corollary \ref{coro1} is proven by replacing ${D}_{\text{avg}}$ in the proof of Lemma \ref{lem1} with any $f\in\mathcal{D}_{\text{sym}}$.
\end{proof}


\ifreport
\begin{proof}[Proof of Lemma \ref{lem2}]
\else
\begin{proof}[of Lemma \ref{lem2}]
\fi

First, fix the sequence of task completion times such that $\bm{T}(P')=\bm{T}(\pi)=\bm{t}$ for all $\pi\in\Pi$. Using condition 2 and the sample-path optimality of the preemptive earliest due date (EDD) discipline \cite{Jackson55}, one can obtain that for all $\pi\in\Pi$ and $\bm{t}\geq\bm{0}$
\begin{align}
[L_{\max}(\bm{C}(P'))|\bm{T}(P')=\bm{t}] \leq[L_{\max}(\bm{C}(\pi))|\bm{T}(\pi)=\bm{t}].\nonumber
\end{align} 
In addition, one can show that $[L_{\max}(\bm{C}(P')) | \bm{T}(P')=\bm{t}]$ is increasing in $\bm{t}$. Hence,
\begin{align}\label{eq_lem2_order1}
[L_{\max}(\bm{C}(P'))|\bm{T}(P')=\bm{t}] \leq[L_{\max}(\bm{C}(\pi))|\bm{T}(\pi)=\bm{t}'],
\end{align} 
whenever $\bm{0}\leq\bm{t}\leq \bm{t}'$. On the other hand, condition 1 tells us that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}\label{eq_lem2_order2}
[\bm{T}(P')|\mathcal{I}] \leq_{\text{st}}[\bm{T}(\pi)|\mathcal{I}].
\end{align} 
Using \eqref{eq_lem2_order1}, \eqref{eq_lem2_order2}, Theorem 6.B.3, and Theorem 6.B.16(c) of \cite{StochasticOrderBook}, yields that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}\label{eq_lem2_order3}
[L_{\max}(\bm{C}(P'))|\mathcal{I}] \leq_{\text{st}}[L_{\max}(\bm{C}(\pi))|\mathcal{I}].
\end{align} 
Using condition 3, the fact that $L_{\max}$ is increasing, and Theorem 6.B.16(a) of \cite{StochasticOrderBook}, we can obtain 
\begin{align}\label{eq_lem2_order4}
[L_{\max}(\bm{U}(P))|\mathcal{I}]\leq_{\text{st}} [L_{\max}(\bm{C}(P'))|\mathcal{I}].
\end{align} 
Combining \eqref{eq_lem2_order3} and \eqref{eq_lem2_order4}, \eqref{eq_lem2_1} follows. If condition 3 is replaced by $P'=P$, then 
\eqref{eq_lem2_2} follows from \eqref{eq_lem2_order3}. This completes the proof.
\end{proof}
\ifreport
\begin{proof}[Proof of Corollary \ref{coro2}]
\else
\begin{proof}[of Corollary \ref{coro2}]
\fi
We need the rearrangement partial ordering $\leq^{\text{a}}$ defined in \cite[Sec. 6.F]{Marshall2011}: Consider two $n$-vector $\bm{x}$ and $\bm{y}$, $\bm{x}$ is said to \emph{immediately precede} $\bm{y}$ by one pairwise interchange, denote $\bm{x}<^{\text{p}}\bm{y}$, if for some index $i$, $1\leq i\leq n-1$,
\begin{align}
y_i<y_{i+1}, ~x_i= y_{i+1}, ~x_{i+1}=y_i, ~x_l= y_l,~l\neq i,i+1.\nonumber
\end{align}
Let $\leq^{\text{b}}$ denote the ordering of successive interchanges, such that $\bm{x}\leq^{\text{b}}\bm{y}$ if $\bm{x}=\bm{y}$ or if there exists a finite chain $\bm{z}^1,\ldots,\bm{z}^k$ of permutations such that
\begin{align}
\bm{x}<^{\text{p}}\bm{z}^1<^{\text{p}}\ldots<^{\text{p}}\bm{z}^k<^{\text{p}}\bm{y}.\nonumber
\end{align}
Suppose that $\bm{x}$ is a permutation of $\bm{u}$ and $\bm{y}$ is a permutation of $\bm{v}$ such that $\bm{x}_{\uparrow}=\bm{u}_{\uparrow}$ and $\bm{y}_{\uparrow}=\bm{v}_{\uparrow}$. Then, $(\bm{x},\bm{y})\leq^{\text{a}} (\bm{u},\bm{v})$ if there exists permutation matrices $W$ and $U$ such that
\begin{align}
\bm{x}W = \bm{u} U=\bm{x}_{\uparrow},~~~\text{and}~~ \bm{y} W \leq^{\text{b}} \bm{v} U.\nonumber
\end{align}
Hence, one can obtain
\begin{align}
(\bm{x}_{\uparrow},\bm{y}_{\downarrow})\leq^{\text{a}}(\bm{x},\bm{y})\leq^{\text{a}}(\bm{x}_{\uparrow},\bm{y}_{\uparrow}).\nonumber
\end{align}
The following rearrangement inequality is an immediate consequence of Theorem F.14 in Chapter 6 of \cite{Marshall2011}:
\begin{lemma}\label{lem_coro_2}
If \emph{$(\bm{x},\bm{y})\geq^{\text{a}} (\bm{u},\bm{v})$}, then
\begin{align}
\bm{x}-\bm{y}\prec \bm{u}-\bm{v}.\nonumber
\end{align}
\end{lemma}

Now, we are ready to prove Corollary \ref{coro2}. As before, we first fix the sequence of task completion times such that $\bm{T}(P')=\bm{T}(\pi)=\bm{t}$ for all $\pi\in\Pi$. Since $k_1=\ldots=k_n=1$, $\bm{C}(P')$ and $\bm{C}(\pi)$ are permutations of $\bm{t}$. According to condition 2 of Lemma \ref{lem2}, each completed job of policy $P'$ has the smallest due time $d_i$ among all unfinished jobs in the queue. Hence,
\begin{align}
[(\bm{C}(P'), \bm{d}) |\bm{T}(P')=\bm{t}] \geq^{\text{a}} [(\bm{C}(\pi), \bm{d}) |\bm{T}(\pi)=\bm{t}].\nonumber
\end{align}
Then, Lemma \ref{lem_coro_2} tells us that for all $\pi\in\Pi$
\begin{align}\label{eq_coro2_4}
&[\bm{L} (P') |\bm{T}(P')=\bm{t}]\nonumber\\
=&[\bm{C}(P') - \bm{d}|\bm{T}(P')=\bm{t}]\nonumber\\
\prec& [\bm{C}(\pi) - \bm{d}|\bm{T}(\pi)=\bm{t}] \nonumber\\
=&[\bm{L}(\pi)|\bm{T}(\pi)=\bm{t}]. 
\end{align} 
%it is easy to show that $t_{i}\leq {C}_{(i)}(\pi)$ for all $i=1,2,\ldots, n$ and $\pi\in\Pi$. Using condition 2 of Lemma \ref{lem2}, we can obtain that for all $\pi\in\Pi$
%\begin{align}\label{eq_coro2_1}
%[\bm{C}_{\uparrow}(P')|\bm{T}(P')=\bm{t}] = (t_1,t_{2},\ldots,t_{n}) \leq [\bm{C}_{\uparrow}(\pi)|\bm{T}(\pi)=\bm{t}].
%\end{align} 
%On the other hand, the rearrangement inequality \cite[Theorem F.14 of Sec. 6]{Marshall2011} implies that for all $\pi\in\Pi$
%\begin{align}\label{eq_coro2_2}
%\bm{C}_{\uparrow}(\pi) - \bm{d}_{\uparrow} \prec \bm{C}(\pi) - \bm{d}.
%\end{align} 
%In addition, condition 2 of Lemma \ref{lem2} tells us that the jobs are completed in the increasing order of $\bm{d}$. Hence, the job completed at time $C_{(i)}(P')$ has a due time $d_{(i)}$ for all $i=1,\ldots,n$. This implies
%\begin{align}\label{eq_coro2_3}
%\bm{L}_{\uparrow} (P')= \bm{C}_{\uparrow}(P') - \bm{d}_{\uparrow}.
%\end{align} 
%Combining \eqref{eq_coro2_1}-\eqref{eq_coro2_3}, yields for all $\pi\in\Pi$
%\begin{align}\label{eq_coro2_4}
%&[\bm{L}_{\uparrow} (P') |\bm{T}(P')=\bm{t}]\nonumber\\
%=&[\bm{C}_{\uparrow}(P') - \bm{d}_{\uparrow}|\bm{T}(P')=\bm{t}]\nonumber\\
%\leq&[\bm{C}_{\uparrow}(\pi)- \bm{d}_{\uparrow}|\bm{T}(\pi)=\bm{t}]\nonumber\\
%\prec& [\bm{C}(\pi) - \bm{d}|\bm{T}(\pi)=\bm{t}] \nonumber\\
%=&[\bm{L}(\pi)|\bm{T}(\pi)=\bm{t}]. 
%\end{align} 
For any $f\in\mathcal{D}_{\text{Sc}}$, define $g(\bm{x})=f(\bm{x}+\bm{d})$. Then, $g$ is Schur convex. For $\pi\in\Pi$, we can obtain
\begin{align}
&[f(\bm{C} (P')) |\bm{T}(P')=\bm{t}]\nonumber\\
=&[g(\bm{L} (P') ) |\bm{T}(P')=\bm{t}]\nonumber\\
\leq&[g(\bm{L} (\pi)) |\bm{T}(\pi)=\bm{t}]\nonumber\\
=&[f(\bm{C} (\pi)) |\bm{T}(\pi)=\bm{t}],\nonumber
\end{align}
where the inequality is due to \eqref{eq_coro2_4} and the definition of Schur convex functions. The remaining proof is the same as \eqref{eq_lem2_order1}-\eqref{eq_lem2_order4}, where we will need to use the fact that $f$ is increasing.
\end{proof}

%\begin{proof}[of Lemma \ref{thm1}]
%
%\end{proof}
%
%\begin{proof}[of Lemma \ref{thm3}]
%Let $[L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,$ $\ldots, t_J)]$ denote the maximum lateness of policy $\pi$ for given parameters $\mathcal{I}$ and task completion instants $(t_1,\ldots, t_J)$. According to the sample-path optimality of the preemptive Earliest Due Date (EDD) discipline \cite{Jackson55}, $[L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,$ $t_{J,\pi}) = (t_1,\ldots, t_J)]$ is minimized among all policies in $\Pi$, if each completed task belongs to the job with the earliest due date. By condition 2, policy $R$ satisfies this requirement, and hence
%\begin{align}
%&~~~[L_{\max,R} | \mathcal{I}, (t_{1,R},\ldots,t_{J,R}) = (t_1,\ldots, t_J)] \nonumber\\
%&\leq [L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)],~\forall~\pi\in\Pi.\nonumber
%\end{align}
%%Further, $[L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)]$ is an increasing function of $(t_1,\ldots, t_J)$, because if task completions are postponed, the job completions are also postponed. 
%The remaining proof steps are the same with Theorem \ref{thm1}.
%%Therefore, for all $\pi\in\Pi$, we have
%%\begin{align}\label{eq_order2}
%%&~~~~[L_{\max,R} | \mathcal{I}, (t_{1,R},\ldots,t_{J,R}) = (t_1,\ldots, t_J)] \nonumber\\
%%&\leq [L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1',\ldots,t_J')],\nonumber\\
%%&~~~~~~~~~~~~~~~~~~~~\text{whenever}~(t_1,\ldots, t_J)\leq (t_1',\ldots,t_J').
%%\end{align}
%%Using condition 1, \eqref{eq_order2}, and the proof arguments of Theorem 6.B.3 of \cite{StochasticOrderBook}, we can obtain that  for all $\pi\in\Pi$
%%\begin{align}\label{eq_order3}
%%(L_{\max,R},t_{1,R},t_{2,R},\ldots) \leq_{\text{st}} (L_{\max,\pi}, t_{1,\pi},t_{2,\pi},\ldots).
%%\end{align}
%%Then, \eqref{eq_thm3} follows from \eqref{eq_order3} and Theorem 6.B.16 (c) of \cite{StochasticOrderBook}. Finally, \eqref{eq_thm3_1} follows from \eqref{eq_thm3} and Eq (6.B.4) of \cite{StochasticOrderBook}.
%\end{proof}



%\begin{proof}[of Lemma \ref{thm4}]
%The proof steps are the same with Theorem \ref{thm2}.
%\end{proof}

\ifreport
\begin{proof}[Proof of Lemma \ref{lem3}]
\else
\begin{proof}[of Lemma \ref{lem3}]
\fi
Using \eqref{eq_lem3_1} and $\bm{U}(\pi)\leq\bm{C}(\pi)$, we can obtain $[\bm{U}(P)|\mathcal{I}] \leq_{\text{st}} [\bm{C}(\pi)|\mathcal{I}]$ for all $\pi\in\Pi_{PL}$. By this, Theorem 6.B.4.(a) of \cite{StochasticOrderBook}, and the fact that $f$ is increasing, \eqref{eq_lem3_2} follows. This completes the proof.
\end{proof}

==> appendices_2.tex <==


\section{Proofs of Theorem~1 and Corollary 3} \label{app1}
\subsection{Proof of {\large \eqref{eq_delaygap1}} in Theorem \ref{thm1}} \label{sec_app_thm1_1}
We prove \eqref{eq_delaygap1} by using the sufficient conditions in Lemma \ref{lem1} and Corollary \ref{coro1}. The proof steps are as follows:

{\bf Construction of Policy $P'$:}
We construct an {infeasible} policy $P'$. \emph{First, in policy $P'$, all servers are busy whenever the queue is not empty.} If the number of tasks is less than $m$, some tasks are replicated over multiple servers. 
\emph{Second, the task completion times of policy $P'$ are constructed as if there is no task cancellations.} Suppose that at any time $t$, server $l$ has processed a task for $\tau$ seconds, and another copy of this task is completed at time $t$ on another server. In policy $P'$, server $l$ will cancel this task and process a new task. More specifically, in policy $P'$, server $l$ will not process the new task from scratch; instead, it is assumed that the new task assigned to server $l$ has already been processed for $\tau$ seconds by time $t$ (which is infeasible),~and server $l$ will serve the task from this progress point. If two task copies are completed at the same time on two servers, they are assumed to be distinct tasks, instead of two replicated copy of the same task. 
\emph{Finally, the completed tasks of policy $P'$ are relabelled such that each completed task is from the job with the fewest remaining tasks}. (This relabeling operation might be infeasible, because the tasks from different jobs may be simultaneously processed on parallel servers.) 
By this, policy $P'$ is constructed.


%\emph{In policy $P'$, all servers are working whenever the queue is not empty, and task cancellations do not affect the task completion times in policy $P'$.} More specifically, if the number of remaining tasks is larger than 0 and less than the number of servers $m$, some of the tasks are replicated over multiple servers to make sure that all servers are working. 

%In both policy $P'$ and FUT-NR, all servers are busy whenever the queue is not empty. 
%
%Suppose that at any time $t$, server $l$ has processed a task for $\tau$ seconds, and another copy of this task is completed at time $t$ on another server. In FUT-NR, after canceling the task with some delay overhead, server $l$ will process a new task that have not been served. 
%%In policy $P'$, task cancellations are implemented for two cases: If server $l$ is an NWU server, server $l$ will process a new task that have not been served (the same as FUT-NR). If server $l$ is an NBU server, 
%In policy $P'$, server $l$ will not process a new task from scratch; instead, it is assumed that at time $t$, the next task assigned to server $l$ is already processed for $\tau$ seconds by a genie (which is infeasible!) and server $l$ will serve the task from this progress point. Therefore, in policy $P'$, the task completion times of NBU servers are constructed as if there is no task cancellations. Finally, the completed tasks in policy $P'$ are relabelled such that each completed task is from the job with the fewest remaining tasks (which is also infeasible, because the tasks from different jobs are processed simultaneously). Note that both policy $P'$ and FUT-NR are work-conserving.

Next, we prove the conditions of Lemma \ref{lem1} one by one.

\textbf{Condition 1:} \emph{Policy $P'$ is more {work-efficient} than any policy $\pi\in\Pi$}. 
%Recall that $\bm{T}(\pi)=(T_1(\pi),\ldots, T_{k_{\text{sum}}}(\pi))$ is the sequence of task completion times of the system. 
\ifreport
\begin{proof}[Proof of Condition 1]
\else
\begin{proof}[of Condition 1]
\fi
We prove condition 1 by induction. Consider the first task completion time $T_1(\pi)$. Job 1 arrives at time $a_1=0$. 
If policy $\pi$ is non-preemptive and work-conserving, then
\begin{align}
[T_1(\pi)|\mathcal{I}]=\min_{l=1,\ldots,m} X_l.\nonumber
\end{align} 
If policy $\pi$ is preemptive and work-conserving, then some  servers may cancel the current task and switch to process a new task at time $t\in[0,T_1(\pi))$, then Lemma \ref{lem_property_MNBUMNWU} tells us that
\begin{align}\label{eq_condition1_2_1}
\min_{l=1,\ldots,m} X_l \leq_{\text{st}}[T_1(\pi)|\mathcal{I}].
\end{align}
If policy $\pi$ is non-work-conserving, then \eqref{eq_condition1_2_1} still holds, because of the possibility of server idleness. Since policy $P'$ is non-preemptive and work-conserving, we can obtain that for all $\pi\in\Pi$
\begin{align}\label{eq_condition1_2}
[T_1(P')|\mathcal{I}]=\min_{l=1,\ldots,m} X_l\leq_{\text{st}}[T_1(\pi)|\mathcal{I}].
\end{align} 



Next, consider the update from $T_j(\pi)$ to $T_{j+1}(\pi)$. Recall that $s_j$ is the $j$-th task arrival time of the system. If $s_{j+1}>T_j(\pi)$, the first $j$ tasks are completed before the $(j+1)$-th task arrives, hence all servers are idle during $[T_j(\pi),s_{j+1})$; otherwise, if $s_{j+1}\leq T_j(\pi)$, the servers can keep working after $T_j(\pi)$. For any work-conserving policy $\pi$, we can obtain
\begin{eqnarray}\label{eq_thm1_2}
T_{j+1}(\pi)\!=\max\{s_{j+1},T_j(\pi)\} + \!\min_{l=1,\ldots,m} R_{j,l}(\pi),
\end{eqnarray}
where $R_{j,l}(\pi)$ is the time duration for server $l$ to complete a task after time $\max\{s_{j+1},T_j(\pi)\}$. 



Suppose that $s_{j+1}\leq T_j(\pi)$ and server $l$ has spent $\tau_l$ ($\tau_l\geq0$) seconds on a task by time $T_j(\pi)$. 
In policy $P'$,  the task completion times are constructed as if there is no task cancellations. Hence, the tail probability for the servers to complete a task after time $T_j(P')$ is 
\begin{align}\label{eq_thm1_7}
&\Pr\Big[\min_{l=1,\ldots,m} R_{j,l}(P')>t\Big]\nonumber\\
=& \Pr\Big[\min_{l=1,\ldots,m}(X_l-\tau_l)>t\Big|\bm{X}> \bm{\tau} \Big].
\end{align}
If $\pi$ is a non-preemptive work-conserving policy, some servers may cancel the tasks they are processing  at time $T_j(\pi)$. If the servers in $\mathcal{S}^c$ cancel the current task and switch to process a new task at time $T_j(\pi)$, then the tail probability for the servers to complete a task after time $T_j(\pi)$ is 
\begin{align}\label{eq_thm1_8}
&\Pr\Big[\min_{l=1,\ldots,m} R_{j,l}(\pi)>t\Big]\nonumber\\
=&\Pr\!\Big[\min\Big\{\min_{l\in\mathcal{S}}(X_l-\tau_l),\min_{l\in\mathcal{S}^c}X_l\Big\}\!>t \Big| \bm{X}_{\mathcal{S}}> \bm{\tau}_{\mathcal{S}}\Big].
\end{align} 
Combining \eqref{eq_thm1_7}, \eqref{eq_thm1_8}, and Lemma \ref{lem_property_MNBUMNWU}, yields 
\begin{align}\label{eq_min}
\min_{l=1,\ldots,m} R_{j,l}(P') \leq_{\text{st}} \min_{l=1,\ldots,m} R_{j,l}(\pi).
\end{align}
If $\pi$ is a preemptive work-conserving policy, then some servers may cancel the current task and switch to process a new task at a particular time $t\in[T_j(\pi),T_{j+1}(\pi))$.
In this case, we can use Lemma \ref{lem_property_MNBUMNWU} to show that \eqref{eq_min} holds. Hence, \eqref{eq_min} holds for all work-conserving policy $\pi$. 

Suppose that $s_{j+1}> T_j(\pi)$, then the servers start to process new tasks at time $s_{j+1}$. In this case, we can show that
\eqref{eq_min} also holds for all work-conserving policy $\pi$. 

Using \eqref{eq_thm1_2}, \eqref{eq_min}, and the fact that $s_j$ is uniquely determined by $\mathcal{I}$, it follows that for all work-conserving policy $\pi$
\begin{align}\label{eq_thm1_4}
[T_{j+1}(P') | \mathcal{I},  T_j(P') = t_j] \leq_{\text{st}} [T_{j+1}(\pi) | \mathcal{I},  T_j(\pi) = t_j'] \nonumber\\
\text{whenever}~ t_j \leq t_j',j=1,2,\ldots
\end{align}
If policy $\pi$ is non-work-conserving, \eqref{eq_thm1_2} becomes
\begin{eqnarray}\label{eq_thm1_2_1}
T_{j+1}(\pi)\!\geq\max\{s_{j+1},T_j(\pi)\} + \!\min_{l=1,\ldots,m} R_{j,l}(\pi),\nonumber
\end{eqnarray}
because of the possibility of server idleness. In this case, \eqref{eq_thm1_4} still holds. Hence, \eqref{eq_thm1_4} holds for all $\pi\in\Pi$.
Then, combining \eqref{eq_condition1_2}, \eqref{eq_thm1_4}, and Theorem 6.B.3 of \cite{StochasticOrderBook}, yields
\begin{align}%\label{eq_thm1_5}
[(T_1(P'),\ldots,T_j(P'))|\mathcal{I}] \leq_{\text{st}} [(T_1(\pi),\ldots,T_j(\pi))|\mathcal{I}],~\forall~\pi\in\Pi.\nonumber
\end{align}
Hence, condition 1 is proven.
\end{proof}

\textbf{Condition 2:} \emph{Each completed task of policy $P'$ belongs to the job with the fewest remaining tasks}. Condition 2 directly follows from the construction of policy $P'$.

\textbf{Condition 3:} \emph{It holds that} 
%\begin{align}
%\mathbb{E}\left[{D}_{\text{avg,FUT-NR}}\right]\leq \mathbb{E}\left[{D}_{\text{avg}}(P')| \mathcal{I}\right] \nonumber\\
%+\frac{1}{N}\sum_{h=1}^N \max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\left[\max_{l\in S} X_l\right].
%\end{align}
\begin{align}\label{eq_condition3}
[\bm{U}_{\uparrow}(\text{FUT-NR})|\mathcal{I}] \leq_{\text{st}} [\bm{C}_{\uparrow}(P')|\mathcal{I}].
\end{align}
We prove condition 3 by a \emph{sample-path ordering} technique, which is motivated by the second proof of the  optimality of SRPT in single-server queueing systems \cite{Smith78}. The generalization from \cite{Smith78} to this {sample-path ordering} technique is non-trivial and unexpected when this research started.


%It is difficult to compare policies $P'$ and FUT-NR directly.~Hence, we will construct an intermediate policy called
%Fewest Positive Unassigned Tasks first with Virtual Tasks (FUT-VT), and prove the following results:
%\begin{align}\label{eq_condition3_1}
%&[{D}_{\text{avg,FUT-NR}}|\mathcal{I}]  \leq_{\text{st}} [{D}_{\text{avg,FUT-VT}}| \mathcal{I}],\\
%&[{D}_{\text{avg,FUT-VT}}|\mathcal{I}]  \leq_{\text{st}} [{D}_{\text{avg}}(P')| \mathcal{I}] + G.\label{eq_condition3_2}
%\end{align}
%Then, \eqref{eq_condition3} follows from \eqref{eq_condition3_1} and \eqref{eq_condition3_2}. 
%
%First, we construct the sample path of policy FUT-VT. In FUT-VT, there are always $m$ virtual tasks in the system, each belongs to a virtual job. Because of these $m$ virtual tasks, the total number of remaining tasks is always no smaller than $m$. Hence, there is no task replications in FUT-VT. In the meanwhile, the task completion times of policy $P'$ are constructed as if there is no task cancellations. Therefore, the task completion sample paths of policies $P'$ and FUT-VT can be aligned (see Fig. \ref{fig_compare} for an illustration): Consider a busy period $[\tau,\nu)$ of policy $P'$. If all $m$ servers start to process new tasks at time $\tau$ in both policies $P'$ and FUT-VT, the task completion times of the two policies are exact the same during the period $[\tau,\nu)$. At time $\nu$, the queue of policy $P'$ is empty, and hence all severs becomes empty.  
%
%An illustration of FUT-NR, FUT-VT, and the lower bound policy $P'$ is provided in .
%
% policy $P'$
%
%On the other hand, there is no virtual task in FUT-NR and hence the servers can spend time to process replicated task copies, instead of wasting time on virtual tasks. By this, \eqref{eq_condition3_1} follows. 
%
%Next, we compare policies $P'$ and FUT-VT. Consider the completion times $(T_1(\pi),\ldots,T_j(\pi))$ of the first $J$ tasks in policies $P'$ and FUT-VT. Note that virtual tasks are completed in FUT-VT, which is not counted in job completion time. We will show that 
%\begin{align}
%[(t_{1,\text{FUT-VT}},\ldots,t_{J,\text{FUT-VT}})|\mathcal{I}] \leq_{\text{st}} [(T_1(P'),\ldots,T_j(P'))|\mathcal{I}].
%\end{align}


First, we define the system states of policies $P'$ and FUT-NR. 
\begin{definition}\label{def_state_P}
The system state of  policy $P'$ is specified by an infinite vector $\bm{\beta}=(\beta_1,\beta_2,\ldots)$ with non-negative, non-increasing components. At any time, the coordinates of $\bm{\beta}$ are interpreted as follows: $\beta_1$ is the maximum number of remaining tasks among all jobs in the queue, $\beta_2$ is the next greatest number of remaining tasks among all jobs in the queue, and so on, with duplications being explicitly repeated. If there are $l$ unfinished jobs in the system, then it holds that
\begin{eqnarray}
\beta_1\geq\beta_2\geq\ldots\geq\beta_l>0 = \beta_{l+1} =\beta_{l+2}=\ldots.\nonumber
\end{eqnarray}
\end{definition}

\begin{definition}\label{def_state}
The system state of FUT-NR is specified by a pair of infinite vectors $\bm{\alpha}=(\alpha_1,\alpha_2,\ldots)$ and $\bm{\delta}=(\delta_1,\delta_2,$ $\ldots)$ with non-negative components. At any time, the coordinates of $\bm{\alpha}$ and $\bm{\delta}$ are interpreted as follows: $\alpha_h$ is the number of unfinished tasks of the job associated to the $h$-th coordinate, and $\delta_h$ out of these $\alpha_h$ tasks are being processed on some servers. Hence, 
\begin{align}\label{eq_def_state}
\delta_h \leq \alpha_h\leq k_{\max},~\sum_{h=1}^\infty \delta_h\leq m. 
\end{align}
The coordinates of $\bm{\alpha}$ and $\bm{\delta}$ are sorted in the non-increasing order of $\alpha_h-\delta_h$, with duplications being explicitly repeated. 
%When $\alpha_h-\delta_h=\alpha_{i+1}-\delta_{i+1}$, the coordinates are sorted such that $\alpha_h\geq \alpha_{i+1}$. 
If there are $l$ unfinished jobs in the system, then there exists an integer $r$ ($0\leq r\leq l$) such that 
\begin{eqnarray}
&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\alpha_1-\delta_1\geq\ldots\geq \alpha_{r}-\delta_{r}>0= \alpha_{r+1}-\delta_{r+1}=\ldots,\\
&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\alpha_h \left\{\begin{array}{l l} >0, &\text{if}~ h\leq l;\\
  =0, &\text{if}~ h\geq l+1,\end{array}\right.~~\delta_h \left\{\begin{array}{l l} \geq0, &\text{if}~ h\leq l;\\
  =0, &\text{if}~ h\geq l+1.\end{array}\right.
  \end{eqnarray}
\end{definition}

Let $\{\bm{\beta}(t),t\geq0\}$ be the state process of policy $P'$ and $\{\bm{\alpha}(t),\bm{\delta}(t),t\geq0\}$ be the state process of FUT-NR, which are assumed to be right-continuous. One key result of the sample-path ordering technique is the following lemma:



\begin{lemma}\label{lemG4}
Suppose that $\bm{\alpha}(0^-) = \bm{\delta}(0^-)=\bm{\beta}(0^-)=\bm{0}$ and the job parameters $\mathcal{I}$ are given. For any sample path of policy $P'$, there exists a sample path of FUT-NR with the same probability density such that
\begin{eqnarray}\label{eq_lemG4}
\sum_{h=j}^\infty [\alpha_h(t)- \delta_h(t)]\leq \sum_{h=j}^\infty \beta_h(t)
\end{eqnarray}
holds for all $t\geq0$ and j = $1,2,\ldots$
\end{lemma}

The following lemmas are needed to prove Lemma \ref{lemG4}:

\begin{lemma}\label{lem_non_prmp1}
Suppose that, under policy FUT-NR, $\{\bm{\alpha}',\bm{\delta}'\}$ is obtained by completing a task on one server in the system whose state is $\{\bm{\alpha},\bm{\delta}\}$. Further, suppose that, under policy $P'$, $\bm{\beta}'$ is obtained by completing a task on one server in the system whose state is $\bm{\beta}$.
If
\begin{eqnarray}\label{eq_non_prmp_41}
\sum_{h=j}^\infty [\alpha_h - \delta_h]\leq \sum_{h=j}^\infty \beta_h, ~\forall~j=1,2,\ldots,\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40}
\sum_{h=j}^\infty [\alpha'_h - \delta'_h]\leq \sum_{h=j}^\infty \beta'_h, ~\forall~j=1,2,\ldots
\end{eqnarray}
\end{lemma}

\begin{proof}
The proof is similar to that of Lemma 2 in \cite{Smith78}.
If $\sum_{h=j}^\infty [\alpha'_h - \delta'_h]=0$, then the inequality \eqref{eq_non_prmp_40} follows naturally. 
If $\sum_{h=j}^\infty [\alpha'_h - \delta'_h]>0$, then there exist some tasks that have not been assigned to any server. 
In FUT-NR, a server that has just completed a task will be allocated to process an unassigned task from the job with the minimum positive $\alpha'_h - \delta'_h$. Hence,
$\sum_{h=j}^\infty [\alpha'_h - \delta'_h]=\sum_{h=j}^\infty [\alpha_h - \delta_h] - 1 \leq \sum_{h=j}^\infty \beta_h -1 \leq \sum_{h=j}^\infty \beta'_h$.
\end{proof}


\begin{lemma}\label{lem_non_prmp2}
Suppose that, under policy FUT-NR, $\{\bm{\alpha}',\bm{\delta}'\}$ is obtained by adding a job with $b$ tasks to the system whose state is $\{\bm{\alpha},\bm{\delta}\}$. Further, suppose that, under policy $P'$, $\bm{\beta}'$ is obtained by adding a job with $b$ tasks to the system whose state is $\bm{\beta}$.
If
\begin{eqnarray}
\sum_{h=j}^\infty [\alpha_h - \delta_h]\leq \sum_{h=j}^\infty \beta_h, ~\forall~j=1,2,\ldots,\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{h=j}^\infty [\alpha'_h - \delta'_h]\leq \sum_{h=j}^\infty \beta'_h, ~\forall~j=1,2,\ldots\nonumber
\end{eqnarray}
\end{lemma}

\begin{proof}
The proof is similar to that of Lemma 3 in \cite{Smith78}.
Without loss of generalization, we suppose that after the job arrival, $b$ is the $l$-th coordinate of $\bm{\alpha}'$ and the $m$-th coordinate of $\bm{\beta}'$. Hence, $\alpha'_l = \beta'_m= b$. Because no server completes a task at this time instant, $\delta'_l =0$. We consider the following four cases:

{Case 1}: $l<j, m<j$. We can obtain $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] = \sum_{h=j-1}^\infty [\alpha_h - \delta_h] \leq \sum_{h=j-1}^\infty \beta_h= \sum_{h=j}^\infty \beta_h'$.

{Case 2}: $l<j, m\geq j$. We have $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] =\sum_{h=j-1}^\infty $ $[\alpha_h - \delta_h] \leq b + \sum_{h=j}^\infty [\alpha_h - \delta_h] \leq b + \sum_{h=j}^\infty \beta_h = \sum_{h=j}^\infty \beta_h'$.

{Case 3}: $l\geq j, m<j$. We have $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] = b + \sum_{h=j}^\infty [\alpha_h - \delta_h] \leq \sum_{h=j-1}^\infty [\alpha_h - \delta_h] \leq \sum_{h=j-1}^\infty \beta_h = \sum_{h=j}^\infty \beta_h'$.

{Case 4}: $l\geq j, m\geq j$. We have $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] = b + \sum_{h=j}^\infty [\alpha_h - \delta_h] \leq b + \sum_{h=j}^\infty \beta_h = \sum_{h=j}^\infty \beta_h'$.
\end{proof}


\ifreport
\begin{proof}[Proof of Lemma \ref{lemG4}]
\else
\begin{proof}[of Lemma \ref{lemG4}]
\fi
Consider any busy period $[\tau,\nu)$ of policy $P'$. Then, in policy $P'$, all servers are busy during $[\tau,\nu)$, and are idle at time $\tau^-$ and time $\nu$. We prove \eqref{eq_lemG4} for $t\in[\tau,\nu)$ by considering two cases:

\emph{Case 1: At time $t=\tau^-$, policy FUT-NR has $m$ tasks and the service of these tasks has just started.} Consider the system states of both policies at time $\tau^-$. The system state of policy FUT-NR satisfies 
\begin{align}\label{proof_lemG4_1}
\sum_{h=1}^\infty \alpha_h(\tau^-)= m, ~\bm{\alpha}(\tau^-)=\bm{\delta}(\tau^-).
\end{align}
In policy $P'$, there is no task in the system at time $\tau^-$ such that 
\begin{align}\label{proof_lemG4_5}
\bm{\beta}(\tau^-)=\bm{0}. 
\end{align}
Consider the evolutions of both policies during $[\tau,\nu)$. 
In policy $P'$, all servers are busy if there is at least one task. On the other hand, in policy FUT-NR, there is no task replication. Hence, all servers are busy if there are no less than $m$ tasks. Because the servers become busy in policy $P'$ at time $\tau$, a job must has arrived. By \eqref{proof_lemG4_1} and \eqref{proof_lemG4_5}, it holds that for $t=\tau$
%^there are no less than $m$ tasks in policy FUT-NR at time $\tau^-$.
\begin{align}\label{proof_lemG4_4}
\sum_{h=1}^\infty \alpha_h(t)= \sum_{h=1}^\infty \beta_h(t) +m\geq m+1.
\end{align}
Therefore,  the servers are all busy in policy $P'$ and policy FUT-NR at time $\tau$. Hence, for any sample path of policy $P'$, there is a sample path of policy FUT-NR such that for sufficiently small $\Delta t$ the task arrival times and task completion times of the two policies are exactly the same during $[\tau,\tau+\Delta t)$, and \eqref{proof_lemG4_4} holds during $[\tau,\tau+\Delta t)$. By induction over time, we can show that for any sample path of policy $P'$, there is a sample path of policy FUT-NR with the same probability density such that the task arrival times and task completion times of the two policies are exactly the same  during $[\tau,\nu)$, and \eqref{proof_lemG4_4} holds for all $t\in[\tau,\nu)$. Using Lemma \ref{lem_non_prmp1}, Lemma \ref{lem_non_prmp2}, and the initial states at time $\tau^-$, we can prove that \eqref{eq_lemG4} holds for all $t\in[\tau,\nu)$ on these two sample paths.

%In general, suppose that at some time $t\in[\tau,\nu)$
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t)= \sum_{h=1}^\infty \beta_h(t) +m\geq m+1.\nonumber
%\end{align}
%Then, the scheduling decisions of policies $P'$ and policy FUT-NR are the same at time $t$. This further implies that for any sample path of policy $P'$, we can construct a sample path of policy FUT-NR such that 
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t^+)= \sum_{h=1}^\infty \beta_h(t^+) +m\geq m+1.\nonumber
%\end{align}
%Therefore, 
%
%Using Lemma \ref{lem_non_prmp1} and Lemma \ref{lem_non_prmp2}, and we can prove that 
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t^+)= \sum_{h=1}^\infty \beta_h(t^+) +m.\nonumber
%\end{align}
%
%For any sample path of policy $P'$ during $[\tau,\nu)$, we can construct a sample path of policy FUT-NR during $[\tau,\nu)$ with the same probability density such that the task arrival times and task completion times of the two policies are exactly the same. In particular, if 
%
%
%if policy $P'$ has $b$ tasks at time $t\in[\tau,\nu)$, policy FUT-NR has $m+b$ tasks at time $t$. Hence, the scheduling decisions of policies $P'$ and policy FUT-NR are the same at time $t$. Therefore, we can obtain
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t)= \sum_{h=1}^\infty \beta_h(t) +m,~\forall~t\in [\tau,\nu).\nonumber
%\end{align}
%Because the task arrivals and departures of policies $P'$ and FUT-NR are aligned during $[\tau,\nu)$, using Lemma \ref{lem_non_prmp1}, Lemma \ref{lem_non_prmp2}, and the initial states at time $\tau^-$, we can prove by induction that \eqref{eq_lemG4} holds for $t\in[\tau,\nu)$.

\emph{Case 2: At time $t=\tau^-$, policy FUT-NR has less than $m$ tasks or the service of these tasks started before time $\tau^-$}. In both \emph{Case 1} and \emph{Case 2}, the sample path evolutions of policy $P'$ are the same. On the other hand, in policy FUT-NR, the tasks are completed earlier in \emph{Case 2} than in \emph{Case 1}. Therefore, \eqref{eq_lemG4} also holds in \emph{Case 2} for $t\in[\tau,\nu)$.

%Note that the case that policy FUT-NR has more than $m$ tasks at time $\tau^-$ will not happen. This will be clear 
Let $[\tau_1,\nu_1)$ be the next busy period of policy $P'$ with $\nu<\tau_1$. Then, $[\nu,\tau_1)$ is an idle period of policy $P'$. We prove \eqref{eq_lemG4} during the idle period $[\nu,\tau_1)$. 
Because all servers are idle during $[\nu,\tau_1)$ in policy $P'$, it follows that 
\begin{align}\label{proof_lemG4_2}
\bm{\beta}(t)=\bm{0},~t\in[\nu,\tau_1).
\end{align}
Hence, there is no task arrival during $[\nu,\tau_1)$; otherwise, \eqref{proof_lemG4_2} cannot be true.
On the other hand, at time $\nu$ there are no more than $m$ tasks in policy FUT-NR such that 
\begin{align}
\bm{\alpha}(\nu)=\bm{\delta}(\nu).\nonumber
\end{align}
Because there is no task arrival during $[\nu,\tau_1)$, policy FUT-NR satisfies
\begin{align}\label{proof_lemG4_3}
\bm{\alpha}(t)=\bm{\delta}(t),~t\in[\nu,\tau_1).
\end{align}
By \eqref{proof_lemG4_2} and \eqref{proof_lemG4_3}, \eqref{eq_lemG4} holds during $[\nu,\tau_1)$.
Further, from \eqref{proof_lemG4_3}, we can obtain
\begin{align}
\sum_{h=1}^\infty \alpha_h(\tau_1^-)=\sum_{h=1}^\infty \delta(\tau_1^-)\leq m,
\end{align}
such that there are no more than $m$ tasks at time $t=\tau_1^-$ in policy FUT-NR. Hence, either \emph{Case 1} or \emph{Case 2} is satisfied at time $t=\tau_1^-$. Then, we can use the above arguments to prove that  \eqref{eq_lemG4} holds during the next busy period $[\tau_1,\nu_1)$ of policy $P'$.


Finally, by taking an induction over the busy and idle periods of policy $P'$,  Lemma \ref{lemG4} is proven.
%Let $[\nu,\tau_1)$ and $[\tau_1,\nu_1)$ be the next idle and busy periods of policy $P'$, respectively. Because policy $P'$ is work-conserving, all $m$ servers are idle in policy $P'$ during $[\nu,\tau_1)$. Hence, there is no job arrival during $[\nu,\tau_1)$. At time $\nu$, we have
%\begin{align}
%\sum_{h=j}^\infty [\alpha_h(\nu)- \delta_h(\nu)]\leq 0.\nonumber
%\end{align}
%This and $\alpha_h(\nu)\geq\delta_h(\nu)$ imply that $\alpha_h(\nu)=\delta_h(\nu)$ for all $h=1,2,\ldots$ Since no job arrives during $[\nu,\tau_1)$, we can obtain that $\alpha_h(t)=\delta_h(t)$ for all $t\in[\nu,\tau_1)$ and $h=1,2,\ldots$ Hence, \eqref{eq_lemG4} holds during $[\nu,\tau_1)$. 
%
%Because there is no job arrival during $[\nu,\tau_1)$, there are no more than $m$ remaining tasks in FUT-NR at time $\tau_1$ and each remaining task has been processed by a certain amount of time. Similar with the case of $[\tau,\nu)$, we can prove that \eqref{eq_lemG4} holds in the busy period $[\tau_1,\nu_1)$.
%By taking an induction over the busy and idle periods of policy $P'$, Lemma \ref{lemG4} follows.
\end{proof}

\ifreport
\begin{proof}[Proof of Condition 3]
\else
\begin{proof}[of Condition 3]
\fi
%Let the evolution of the system state under some scheduling policy be on a space $(\Omega,\mathcal{F},P)$. Each $\omega\in\Omega$ corresponds to a sample path of policy $P'$ and a sample path of policy FUT-NR. The job arrival parameters $\mathcal{I}$ is fixed for all $\omega\in\Omega$. 
%Let $(C_{(1)}(P'),\ldots,c_{N:N}(P'))$ be a permute of the job completion time sequence $(c_{1}(P'),\ldots,c_{N}(P'))$ in the increasing order, such that $c_{i:N}(P')\leq c_{i+1:N}(P')$. 

%Pick any $\omega\in\Omega$ and consider the first job completion time $C_{(1)}(P')$ of policy $P'$. Suppose that there are $y$ job arrivals during $[0,C_{(1)}(P'))$. 

We will prove Condition 3 by induction. Consider the sample paths of policy $P'$ and policy FUT-NR satisfying Lemma \ref{lemG4}. We first show that there exists a job $w_1$ such that
\begin{align}\label{eq_Condition_3_1}
U_{w_1}(\text{FUT-NR}) \leq C_{(1)}(P').
\end{align}

In policy $P'$, the first job departure occurs at time $t=C_{(1)}(P')$. Suppose that $y_1$ jobs have arrived during $[0,C_{(1)}(P'))$. Then, there are $y_1-1$ unfinished jobs at time $C_{(1)}(P')$ in policy $P'$. Hence, the system state of policy $P'$ satisfies 
\begin{align}\label{eq_proof_0}
\sum_{h=y_1}^\infty\beta_h(C_{(1)}(P'))=0.
\end{align}
This and Lemma \ref{lemG4} imply
%Hence, there are $y-1$ unfinished jobs at time $C_{(1)}(P')$ such that
%Invoking Lemma \ref{lemG4}, we can obtain
\begin{align}\label{eq_proof_1}
\sum_{h=y_1}^\infty \alpha_h(C_{(1)}(P'))\leq \sum_{h=y_1}^\infty  \delta_h(C_{(1)}(P')).
\end{align}
In policy FUT-NR, there are at most $y_1$ jobs at time $C_{(1)}(P')$. Hence, the system state of policy FUT-NR must satisfy
\begin{align}\label{eq_proof_2}
\!\!\alpha_h(C_{(1)}(P'))= \delta_h(C_{(1)}(P'))=0,\forall~h=y_1\!+\!1,y_1\!+\!2,\ldots \!\!
\end{align}
Combining \eqref{eq_proof_1}, \eqref{eq_proof_2}, and the fact that $\alpha_h(t)\geq\delta_h(t)$ for all $h$ and $t$, we can obtain
%Combining \eqref{eq_proof_0}, \eqref{eq_proof_1}, and the fact that $\alpha_h(t)\geq\delta_h(t)$ for all $i,t$, yields
\begin{align}\label{eq_proof_3}
\alpha_{y_1}(C_{(1)}(P'))=\delta_{y_1}(C_{(1)}(P')).
\end{align}
Let $w_1$ be the index of the job associated to the $y_1$-th coordinate of $\bm{\alpha}(t)$ at time $t= C_{(1)}(P')$. Then, \eqref{eq_proof_3} tells us that in FUT-NR, all tasks of job $w_1$ are either completed or under service at time $C_{(1)}(P')$. Hence, \eqref{eq_Condition_3_1} is proven.
%\begin{align}%\label{eq_proof_9}
%U_{w_1}(\text{FUT-NR}) \leq C_{(1)}(P'),\nonumber
%\end{align}
%which implies \eqref{eq_Condition_3_1}.

Next, we prove the induction step. Suppose that there exist $j$ jobs indexed by $w_1,w_2,\ldots,w_j$ such that
\begin{align}
U_{w_i}(\text{FUT-NR}) \leq C_{(i)}(P'),~i=1,\ldots,j,\nonumber
\end{align}
we will show that there exist another job $w_{j+1}$ such that
\begin{align}\label{eq_proof_9}
U_{w_{j+1}}(\text{FUT-NR}) \leq C_{(j+1)}(P').
\end{align}
%Since preemption is not allowed, these $\delta_y(C_{(1)}(P'))$ tasks will be under service in policy FUT-NR until completion. Let $w_1$ be the index of the job associated to the coordinate $y$ at time $C_{(1)}(P')$. According to \eqref{eq_def_state}, we can obtain $\delta_y(C_{(1)}(P'))\leq \min[k_{w_1},M].$ Therefore, the time duration between $C_{(1)}(P')$ and $c_{w_1,\text{FUT-NR}}$ is no more than the time to complete $\min[k_{w_1},M]$ tasks of job $w_1$.
Assume that $y_{j+1}$ jobs have arrived during $[0,C_{(j+1)}(P'))$, which must satisfy $y_{j+1}\geq j+1$. Then, 
there are $(y_{j+1}-j-1)$ unfinished jobs at time $C_{(j+1)}(P')$ in policy $P'$. According to \emph{Definition \ref{def_state_P}}, the system state of policy $P'$ satisfies 
\begin{align}
\sum_{h=y_{j+1}-j}^\infty\beta_h(C_{(j+1)}(P'))=0.\nonumber
\end{align}
Then, by following the arguments of \eqref{eq_proof_1}-\eqref{eq_proof_3}, we can obtain that at time $t=C_{(j+1)}(P')$ the system state of policy FUT-NR satisfies
\begin{align}\label{eq_proof_4}
\alpha_{h}(C_{(j+1)}(P'))=\delta_{h}(C_{(j+1)}(P')),~h=y_{j+1}-j,\ldots,y_{j+1}.
\end{align}
There are $j+1$ jobs satisfying \eqref{eq_proof_4}. At least one of these $j+1$ jobs is different from the jobs $w_1,w_2,\ldots,w_j$. Let $w_{j+1}$ be the index of this job. Then, \eqref{eq_proof_4} tells us that in FUT-NR, all tasks of job $w_{j+1}$ are either completed or under service at time $t=C_{(j+1)}(P')$. Hence, \eqref{eq_proof_9} is proven.

By induction, we can obtain
\begin{align}\label{eq_proof_10}
U_{w_{j}}(\text{FUT-NR}) \leq C_{(j)}(P'),~j=1,\ldots,n.
\end{align}
Because $U_{(j)}(\pi)$ is the $j$-th smallest components of $\bm{U}(\pi)$, it follows that
\begin{align}\label{eq_proof_11}
U_{(j)}(\text{FUT-NR})\! \leq \!\max_{i=1,\ldots,j}U_{w_{j}}(\text{FUT-NR}),~j=1,\ldots,n.\!\!
\end{align}
Combining \eqref{eq_proof_10} and \eqref{eq_proof_11}, we obtain that for each sample path of policy $P'$, there is a sample path of policy FUT-NR with the same probability density such that 
\begin{align}
\bm{U}_{\uparrow}(\text{FUT-NR}) \leq  \bm{C}_{\uparrow}(P').
\end{align}
Considering all possible sample paths of these two policies, the stochastic ordering result in \eqref{eq_condition3} follows.
%Suppose that for some $j\in\{1,\ldots,N-1\}$, the time duration between $c_{i:N}(P')$ and $c_{w_i,\text{FUT-NR}}$ is no more than the time for the system to complete $\min[k_{w_i},M]$ tasks of job $w_i$ for all $h=1,\ldots, j$, and the job indices $w_1,w_2,\ldots,w_j$ are distinct. We will prove that there is a job $w_{j+1}$ different from $w_1,w_2,\ldots,w_j$ such that the time duration between $C_{(j+1)}(P')$ and $c_{w_{j+1},\text{FUT-NR}}$ is no more than the time to complete $\min[k_{w_{j+1}},M]$ tasks of a job $w_{j+1}$.
%Let $z$ be the number of job arrivals during $[0,C_{(j+1)}(P'))$, which must satsify $z\geq j+1$. By following the arguments of \eqref{eq_proof_1}-\eqref{eq_proof_9}, we can obtain
%\begin{align}\label{eq_proof_4}
%\alpha_{i}(C_{(j+1)}(P'))=\delta_{i}(C_{(j+1)}(P')),~h=z-j,\ldots,z.
%\end{align}
%Since preemption is not allowed, in policy FUT-NR, the remaining tasks of the $(j+1)$ jobs associated to the coordinates $z-j,z-j+1,\ldots,z$ will be under service after time $C_{(j+1)}(P')$ until completion (or are already completed before time $C_{(j+1)}(P')$). Moreover, at least one of these $(j+1)$ jobs must be different from the jobs $w_1,w_2,\ldots,w_j$. Let $w_{j+1}$ be the index of this job. 
%Using \eqref{eq_def_state} and \eqref{eq_proof_4}, one can show that the time difference between $c_{(j+1)}(P')$ and $c_{w_{j+1},\text{FUT-NR}}$ is no more than the time duration to complete $\min[k_{w_{j+1}},M]$ tasks of job $w_{j+1}$.
%
%By induction, for all $h=1,\ldots,N$ and all $\omega\in\Omega$, the time difference between $c_{i:N}(P')$ and $c_{w_{i},\text{FUT-NR}}$ is no more than the time duration to complete $\min[k_{w_i},M]$ tasks of job $w_i$. Further, the job indices $w_1,w_2,\ldots,w_N$ are distinct, such that $(w_1,w_2,\ldots,w_N)$ is a permute of $(1,2,\ldots,N)$.
% This tells us that 
%\begin{align}
%\mathbb{E}\left[c_{w_i,\text{FUT-NR}} - c_{i:N}(P')| \mathcal{I}\right] \leq \max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\left[\max_{l\in S} X_l\right].\nonumber
%\end{align}
%Hence, we have
%\begin{align}\label{eq_proof_5}
%&\mathbb{E}[{D}_{\text{avg,FUT-NR}}-{D}_{\text{avg}}(P')| \mathcal{I}]\nonumber\\
%=&\frac{1}{N}\sum_{h=1}^N\mathbb{E} \left[c_{i,\text{FUT-NR}} - c_{i}(P')| \mathcal{I}\right]\nonumber\\
%=&\frac{1}{N} \sum_{h=1}^N\mathbb{E} \left[c_{w_i,\text{FUT-NR}} - c_{i:N}(P')| \mathcal{I}\right]\nonumber\\
%\leq &\frac{1}{N}\sum_{h=1}^N\max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\left[\max_{l\in S} X_l\right].
%\end{align}
%By this, condition 3 is proven.
\end{proof}
After establishing conditions 1-3 of Lemma \ref{lem1} for policy FUT-NR,  we can use Lemma \ref{lem1} and Corollary \ref{coro1} to obtain \eqref{eq_delaygap1}. This completes the proof.

\subsection{Proof of {\large \eqref{eq_delaygap2}} in Theorem \ref{thm1}} 
The proof of \eqref{eq_delaygap2} is  similar with that of \eqref{eq_delaygap1} in Appendix \ref{sec_app_thm1_1}, except for the following two differences: 

First, policy FUT-NR in Appendix \ref{sec_app_thm1_1} should be replaced by policy FUT-NIR. 


Second, task replications are allowed in policy FUT-NIR, which will introduce some extra delay to cancel the redundant task copies. %It is important to keep the cancellation overhead small. Otherwise, 
If the cancellation overhead is large, the servers might be busy cancelling the redundant task copies, instead of serving new tasks. In this case, Lemma \ref{lemG4} does not hold. Hence, we should keep the cancellation overhead small. In the design of policy FUT-NIR, a task replica is cancelled if the time to cancel the replica is stochastically shorter than the time to complete the replica; otherwise, the replica will not be cancelled. Using this and the extra conditions {$\bm{O}_{\mathcal{S}}\leq_{\text{st}}[\bm{X}_{\mathcal{S}}-\bm{\tau}_{\mathcal{S}}| \bm{X}>\bm{\tau}]$} and  {$\bm{O}_{\mathcal{S}^c}\geq_{\text{st}}[\bm{X}_{\mathcal{S}^c}-\bm{\tau}_{\mathcal{S}^c}| \bm{X}>\bm{\tau}]$}, we can obtain that in policy FUT-NIR the redundant task copies are completed stochastically earlier than processing these task copies until completion. Using this, the proof arguments of Lemma \ref{lemG4} also work for policy FUT-NIR.

\subsection{Proof of Corollary 3}  
Under the conditions of Corollary \ref{coro3}, policy FUT-NR satisfies the following three properties: (i) all $m$ servers are busy at all time $t\in[0,\infty)$, (ii) there is no task replications, and (iii) any completed task is from a job with the fewest remaining task. Therefore, policy FUT-NR is identical with policy $P'$ constructed in Appendix \ref{sec_app_thm1_1}. In addition, because there are at least $m$ remaining tasks at all time $t\in[0,\infty)$, policy FUT-NIR is identical with policy FUT-NR. Then, \eqref{eq_coro3} follows from Lemma \ref{lem1} and Corollary \ref{coro1}. 

%The details are provided in Appendix \ref{app2}.



%\textbf{Condition 4:} $P\in\Pi$. This condition is trivial. Hence, \eqref{eq_delaygap1} follows from Lemma \ref{thm2}.
%
%The remaining task is to prove \eqref{eq_delaygap2}. Since the $X_l$'s are independent NBU random variables with mean $\mathbb{E}[X_l]=1/\mu_l$, by Theorem 3.A.55 of \cite{StochasticOrderBook}, we can obtain
%\begin{align}
%X_l \leq_{\text{icx}} Z_l,~l=1,\ldots,m,\nonumber
%\end{align}
%where $\leq_{\text{icx}}$ is the increasing convex order defined in \cite[Chapter 4]{StochasticOrderBook} and the $Z_l$'s are independent exponential random variables with mean $\mu_l$. By Corollary 4.A.16 of \cite{StochasticOrderBook}, we have 
%\begin{align}
%\max_{l\in S} X_l \leq_{\text{icx}} \max_{l\in S} Z_l,~\forall~S\subseteq\{1,\ldots,m\}.\nonumber
%\end{align}
%Then, Eq. (4.A.1) of \cite{StochasticOrderBook} and $\mu_1\leq \ldots\leq \mu_M$ tell us that  
%\begin{align}
%\!\!\max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\!\left[\max_{l\in S} X_l\right]\!\leq\!\mathbb{E}\!\left[\max_{l=1,\ldots,k_i \wedge M} Z_l\right]\!\leq\!\sum_{l=1}^{k_i \wedge M} \frac{1}{\sum_{m=1}^l \mu_l}.\nonumber
%\end{align}
%This and \eqref{eq_proof_5} imply \eqref{eq_delaygap2}. This completes the proof.




==> appendices_3version2.tex <==
% !TEX root = ./replication.tex

\section{Proofs of Proposition~\ref{coro3_1}} \label{app0_2}
%\ifreport
%\begin{proof}[Proof of Thoerem \ref{lem3}]
%\else
%\begin{proof}[of Thoerem \ref{lem3}]
%\fi
%Thoerem \ref{lem3} follows from Thoerem \ref{lem2} by letting $d_i=a_i$ for all $i$.
%\end{proof}
%\ifreport
%\begin{proof}[Proof of Corollary~\ref{coro3_1}]
%\else
%\begin{proof}[of Corollary~\ref{coro3_1}]
%\fi
%Proposition~\ref{coro3_1} follows from Corollary \ref{coro2} by letting $d_i=a_i$ for all $i$.
%As in the proof of Corollary \ref{coro2}, let $w_i$ denote the index of the job associated with $v_{(i)}(P)$.
%
%We assume that the arrival times $a_1,\ldots, a_n$ of the $n$ jobs are distinct from each other. This does not lose any generality, because if $a_i=a_j$ for two jobs $i$ and $j$, Proposition~\ref{coro3_1} can be proven by first proving for the case $a_i=a_j+\epsilon$ and then taking the limit $\epsilon\rightarrow 0$. 
We take 3 steps to prove Proposition~\ref{coro3_1}:

\emph{Step 1: We show that}  
%Thoerem \ref{lem3} holds if \emph{$D_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$.}
\begin{align}\label{eq_coro2_2_2}
v_{(i)}(P) \leq c_{(i)}(\pi),~i=1,\ldots,n.
\end{align}

In policy $P$, each unassigned task entering the servers is from the job with the earliest arrival time among all jobs with unassigned tasks. Because each job has $k$ tasks, in policy $P$ only the job with the earliest arrival time may have fewer than $k$ unassigned tasks, the other jobs arrived later have exactly $k$ unassigned tasks. Therefore, among all jobs with unassigned tasks, the job with the earliest arrival time is also the job with the fewest unassigned tasks.
Then, \eqref{eq_coro2_2_2} follows from Proposition~\ref{lem1}. 
In addition, we can use Proposition \ref{lem1} to prove that \eqref{eq_coro3_1_1} holds for all $f\in\mathcal{D}_{\text{sym}}$.

The remaining proof is almost identical with \emph{Step 2} and \emph{Step 3} in the proof of Proposition \ref{coro2}, except that $d_i$ should be replaced by $a_i$. 
By this, Proposition~\ref{coro3_1} is proven.
%Because each job has $k$ tasks, a job can have fewer than $k$ unassigned tasks if and only if some of its tasks are under service, which 
%Because each job has $k$ tasks, only the job under service has fewer than $k$ tasks, , 
%at any time in policy $P$, the job with the earliest arrival time is also the job with the fewest unassigned tasks.
%We can utilize Lemma \ref{lem_sample_path_ordering} to show that $v_{w_j}(P) = v_{(j)}(P) \leq c_{(j)}(\pi)$ for all $j=1,\ldots,n$. In addition, 
%According to Corollary \ref{coro1}, the result of Thoerem \ref{lem3} holds if \emph{$D_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$.
%\emph{Step 2: We show that}
%\begin{align}\label{eq_coro3_3}
%\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}.
%\end{align} 
%
%
%
%We construct a policy $\pi'$ based on policy $\pi$: The sequence of job completion times of policy $\pi'$ is a reordering (rearrangement) of that of policy $\pi$. And in policy $\pi'$, each completed job has the earliest arrival time among all jobs in the queue. We note that because each job has $k$ tasks, it is feasible to reordering the job completion times such that the job arrives earlier is completed earlier.
%% this reordering operation leads to a feasible policy $\pi'$. %In particular, suppose that job $i$ has an earlier arrival time than job $j$. Because both job $i$ and job $j$ have $k$ tasks, the system can switch to process job $i$
%%and more unassigned tasks than the other jobs in the queue, then it is infeasible to reorder the sequence of job completion times such that job $i$ is the next completed job.
%Hence, for the constructed policy $\pi'$, one can use the proof argument of Lemma \ref{lemG4_thm3} to show that
%\begin{eqnarray}\label{eq_pi'_3}
%\sum_{i:a_i\leq\tau} \gamma_{i,P}(t)\leq \sum_{i:a_i\leq\tau} \xi_{i,\pi'}(t), ~\forall~\tau\in[0,\infty)
%\end{eqnarray}
%holds for all $t\in[0,\infty)$. The remaining proof is the same with \emph{Step 2} and \emph{Step 3} in the proof of Corollary \ref{coro2}, where $d_i$ is replaced by $a_i$. 
%By this, Corollary~\ref{coro3_1} is proven.
%\end{proof}

%\subsection{Proof of Corollary \ref{coro2}}
%
%
%In the proof of Corollary \ref{coro2}, we need to use the following rearrangement inequality: 
%\begin{lemma} \cite[Theorem 6.F.14]{Marshall2011}\label{lem_rearrangement}
%Consider two $n$-vectors $(x_1,\dots,x_n)$ and $(y_1,\ldots,y_n)$. If $(x_i- x_j)(y_i-y_j)<0$ for some indices $i$ and $j$ where $1\leq i<j\leq n$, then 
%\begin{align}
%&(x_1\!-\!y_1,\ldots,x_j\!-\!y_i,\ldots,x_i\!-\!y_j,\ldots,x_n\!-\!y_n)\nonumber\\
%\prec& (x_1\!-\!y_1,\ldots,x_i\!-\!y_i,\ldots,x_j\!-\!y_j,\ldots,x_n\!-\!y_n).\nonumber
%\end{align}
%\end{lemma}
%\ifreport
%\begin{proof}[Proof of Corollary \ref{coro2}]
%\else
%\begin{proof}[of Corollary \ref{coro2}]
%\fi
%As in the proof of Lemma \ref{lem_sample_path_ordering_thm3}, let $w_i$ denote the index of the job associated with $v_{(i)}(P)$. 
%
%\emph{Step 1: We show that  
%Thoerem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$.}
%%\begin{align}\label{eq_coro2_2}
%%v_{w_i}(P) \leq c_{(i)}(\pi),~i=1,\ldots,n.
%%\end{align}
%
%Because each job has only one task, it holds in policy $P$ that each task allocated to the servers belongs to the job with the fewest unassigned tasks, whenever there exist unassigned tasks in the system. 
%Hence, 
%%we can utilize Lemma \ref{lem_sample_path_ordering} to show that $v_{w_i}(P) = v_{(i)}(P) \leq c_{(i)}(\pi)$ for all $i=1,\ldots,n$. On the other hand, 
%Corollary \ref{coro1} implies that Thoerem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any {$f\in\mathcal{D}_{\text{sym}}$}.

%Suppose that $b_j$ tasks have been assigned to the servers in policy $P$ by time $c_{(j)}(\pi)$. Since each job has only one task, $j$ tasks are completed by time $c_{(j)}(\pi)$ in policy $\pi$. Because policy $P$ is more work-efficient than policy $\pi$, it must hold that at least $j$ tasks are completed during $[0,c_{(j)}(\pi)]$  in policy $P$. Hence, at least $j$ tasks are assigned to the servers during $[0,c_{(j)}(\pi)]$ in policy $P$. Because each job has only one task, it follows that $v_{w_j}(P) \leq c_{(j)}(\pi)$  for all $j=1,\ldots,n$.

%We prove Corollary \ref{coro2} by induction. 

%\emph{Step 2: We show that}
%\begin{align}\label{eq_coro2_3}
%\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}.
%\end{align} 
%
%
%%We show that Thoerem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{Sch-1}}$.} 
%
%We construct two policies $\pi'$ and $\pi''$ based on policy $\pi$: The sequence of job completion times of policy $\pi'$ is a rearrangement (reordering) of that of policy $\pi$, such that for each job $i$ there exists a job $j$ such that $c_i(\pi') = c_j(\pi)$.
%%, i.e., the completion time of any job $i'$ in policy $\pi'$ must be the completion time of some job $i$ in policy $\pi$.
%Furthermore, in policy $\pi'$, each completed job has the earliest due time among all jobs presenting in the queue, such that $c_1(\pi')\leq c_2(\pi') \leq \ldots \leq c_n(\pi')$. Hence, 
%\begin{align}\label{coro2_1}
%c_i(\pi') = c_{(i)}(\pi).
%\end{align}
%On the other hand, the task completion times of policy $\pi''$ is a rearrangement (reordering) of the task completion times of policy $\pi$, and in policy $\pi''$, each completed task belongs to the jobs with the earliest due time among all jobs presenting in the queue. 
%Let $t_i(\pi)$ be the $i$-th smallest task completion time of policy $\pi$, then 
%\begin{align}\label{coro2_2}
%c_i(\pi'') = t_{ik}(\pi).
%\end{align} 
%%i.e., if job $i$ arrives before the completion time of job $j$ and $d_i<d_j$, then job $i$ is completed before job $j$ in policy $\pi'$. 
%%Let $t_i(\pi)$ be the $i$-th smallest task completion time of policy $\pi$. 
%In policy $\pi$, because each job has $k$ tasks, the system must complete at least $k$ tasks before one job is completed, i.e.,
%$c_{(1)}(\pi)\geq t_{k}(\pi)$. In general, the system must complete at least $ik$ tasks before $i$ jobs are completed, i.e., 
%\begin{align}\label{coro2_3}
%c_{(i)}(\pi)\geq t_{ki}(\pi).
%\end{align} 
%By combining \eqref{coro2_1}-\eqref{coro2_3}, we have
%\begin{align}
%c_i(\pi') = c_{(i)}(\pi)\geq t_{ik}(\pi)=c_i(\pi'').
%\end{align}
%We note that policy $\pi''$ is feasible, but policy $\pi'$ is not because 
%
%
%
%
%
%
%
%
%In policy $\pi''$, the task completion times 
%
%
%For this constructed policy $\pi'$, one can use the proof argument of Lemma \ref{lemG4_thm3} to show that
%\begin{eqnarray}\label{eq_pi'}
%\sum_{i:a_i\leq\tau} \gamma_{i,P}(t)\leq \sum_{i:a_i\leq\tau} \xi_{i,\pi'}(t), ~\forall~\tau\in[0,\infty)
%\end{eqnarray}
%holds for all $t\in[0,\infty)$. That is, Lemma \ref{lemG4_thm3}  holds even if policy $\pi$ is replaced by this constructed policy $\pi'$. %Note that if the jobs have more than one tasks, \eqref{eq_pi'} may not hold for the constructed policy $\pi'$.
%%We rearrange the job completion times of policy $\pi$ as follows: Consider any two jobs $i$ and $j$ which simultaneously exist in the queue at some time, i.e., there exists a time $t$ such that $a_i\leq t\leq c_i(\pi)$ and  $a_j\leq t\leq c_j(\pi)$. If $(c_i(\pi)-c_j(\pi))(d_i- d_j)<0$, we interchange the completion times of job $i$ and job $j$. Repeat this procedure until $(c_i(\pi)-c_j(\pi))(d_i- d_j)\geq 0$ is satisfied for any pair of jobs $i$ and $j$ which simultaneously exist in the queue at some time. Hence, after the rearrangement, each completed job has the earliest due time among all jobs in the queue. Let $c_i'(\pi)$ denote the completion time of job $i$ after the rearrangement. 
%
%In the sequel, we will use \eqref{eq_pi'}, Lemma \ref{lem_rearrangement}, and the property of policy $\pi'$ to prove the following two claims:
%\begin{itemize}
%\item[1.] $\bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}$;
%\item[2.] $v_i(P)\leq c_i(\pi')$ for $i=1,\ldots,n$.
%\end{itemize}
%
%
%%Hence, the $i$-th smallest job completion time $c_{(i)}(\pi')$ of policy $\pi'$ is equal to $i$-th smallest job completion time $c_{(i)}(\pi)$ of policy $\pi$, i.e., $c_{(i)}(\pi')=c_{(i)}(\pi)$.
%
%First, we prove claim 1. An alternative construction procedure of policy $\pi'$ is provided as follows: Suppose that in policy $\pi$, two jobs $i$ and $j$ co-exist in the queue at some time $t$, i.e., $a_i\leq t\leq c_i(\pi)$ and  $a_j\leq t\leq c_j(\pi)$. If $(c_i(\pi)-c_j(\pi))(d_i- d_j)<0$, the completion times of job $i$ and job $j$ are interchanged. 
%Repeat this pair-wise interchange operation until $(c_i(\pi)-c_j(\pi))(d_i- d_j)\geq 0$ is satisfied for any pair of jobs $i$ and $j$ which co-exist in the queue at some time. Then, the job completion times of policy $\pi'$ are obtained.
%By using Lemma \ref{lem_rearrangement} for each pair-wise interchange operation during this construction procedure of policy $\pi'$, we can obtain $\bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}$. By this, claim 1 is proven.
%
%
%Next, we prove claim 2 by contradiction. Suppose that
%\begin{align}\label{eq_contradiction_coro2}
%v_{w_j}(P) > c_{w_j}(\pi')
%\end{align} 
%holds for some $j\in\{1,\ldots,n\}$.
%In policy $\pi'$, if job $i$ arrives before time $c_{w_j}(\pi')$ and $d_i<d_{w_j}$, then job $i$ is completed before time $c_{w_j}(\pi')$. Hence, the system state of policy $\pi'$ satisfies 
%\begin{align}
%\sum_{i:d_i\leq d_{w_j}}\xi_{i,\pi'}(c_{w_j}(\pi')) =0,\nonumber
%\end{align}
%where we have used the fact that $d_i\neq d_j$ if $i\neq j$. Combining this with \eqref{eq_pi'}, we can obtain
%%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(\pi)$ such that
%%Invoking Lemma \ref{lemG4}, we can obtain
%\begin{align}\label{eq_proof_1_coro2}
%\sum_{i:d_i\leq d_{w_j}} \gamma_{i,P}(c_{w_j}(\pi'))\leq 0.
%\end{align}
%By the definition of the system state, we have $\gamma_{i,P}(t)\geq0$ for all $i$ and $t$. This and \eqref{eq_proof_1_coro2} tells us that at time $c_{w_j}(\pi')$, the system state of policy $P$ satisfies
%\begin{align}
%\gamma_{w_j,P}(c_{w_j}(\pi'))= 0.\nonumber
%\end{align}
%That is, all tasks of job $w_j$ are either completed or under service by time $c_{w_j}(\pi')$ in policy $P$. Hence, $v_{w_j}(P)\leq c_{w_j}(\pi')$, which contradicts with \eqref{eq_contradiction_coro2}. Therefore, $v_{w_j}(P)\leq c_{w_j}(\pi')$ holds for all $j=1,\ldots,n$. By this, claim 2 is proven.
%
%Now, we use claim 1 and claim 2 to prove \eqref{eq_coro2_3}. In particular,  claim 1 and claim 2 suggest that
%\begin{align}
%\bm{u}(P)-\bm{d}\leq \bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}.
%\end{align}
%By this and Theorem 5.A.9 of \cite{Marshall2011}, \eqref{eq_coro2_3} follows.
%
%
%\emph{Step 3: We use \eqref{eq_coro2_3} to prove Corollary \ref{coro2}.}
%For any $f\in\mathcal{D}_{\text{Sch-1}}$, $f(\bm{x}+\bm{d})$ is Schur convex. 
%According to Theorem 3.A.8 of \cite{Marshall2011}, for all $f\in\mathcal{D}_{\text{Sch-1}}$, 
%\begin{align}
%&f(\bm{u}(P)) \nonumber\\
%= &f[(\bm{u}(P)-\bm{d})+\bm{d}] \nonumber\\
%\leq& f[(\bm{c}(\pi)-\bm{d})+\bm{d}] \nonumber\\
%=& f(\bm{c} (\pi)).\nonumber
%\end{align} 
%By considering all possible sample paths of these two policies, the stochastic ordering result in Corollary \ref{coro2} follows.
%This completes the proof.
%%\end{proof}
%
%\end{proof}
%
%
%%We develop a {sample-path ordering} technique to prove Thoerem \ref{lem3}. The system state of policy $P$ is the same as that in \emph{Definition \ref{def_state_thm3}}, and the system state of policy $\pi$ are the same as that in \emph{Definition \ref{def_state_P_thm3}}. 
%%
%%
%%We assume that the priorities $p_1,\ldots, p_n$ of the $n$ jobs are distinct from each other. This does not lose any generality, because if $p_i=p_j$ for two jobs $i$ and $j$, Thoerem \ref{lem3} can be proven by taking the limit $p_i\rightarrow p_j$.  The first part of the sample-path ordering result is as follows:
%% 
%% 
%%\begin{lemma}\label{lemG4_lem3}
%%Suppose that $\bm{\gamma}(0^-)=\bm{\zeta}(0^-)=\bm{\xi}(0^-)=\bm{0}$ and the conditions of Thoerem \ref{lem3} are satisfied. Then, the following relationship holds on sample path:
%%\begin{eqnarray}\label{eq_lemG4_lem3}
%%\sum_{i: p_i\geq p} [\gamma_i(t) - \zeta_i(t)]\leq \sum_{i: p_i\geq p} \xi_i(t), ~\forall~p\geq 0.
%%\end{eqnarray}
%%holds for all $t\geq0$.
%%\end{lemma}
%%
%%The following two lemmas are needed to prove Lemma \ref{lemG4_lem3}:
%%
%%
%%\begin{lemma}\label{lem_non_prmp1_lem3}
%%Suppose that, under policy $P$, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by allocating $b$ unassigned tasks to the servers in the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that, under policy $\pi$, $\bm{\xi}'$ is obtained by completing $b'$ tasks in the system whose state is $\bm{\beta}$.
%%If $b\geq b'$ and
%%\begin{eqnarray}
%%\sum_{i: p_i\geq p} [\gamma_i - \zeta_i]\leq \sum_{i: p_i\geq p} \xi_i, ~\forall~p\geq 0,\nonumber
%%\end{eqnarray}
%%then
%%\begin{eqnarray}\label{eq_non_prmp_40_lem3}
%%\sum_{i: p_i\geq p} [\gamma_i'- \zeta_i']\leq \sum_{i: p_i\geq p} \xi_i', ~\forall~p\geq 0.\end{eqnarray}
%%\end{lemma}
%%
%%\begin{proof}
%%If $\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']=0$, then the inequality \eqref{eq_non_prmp_40_lem3} follows naturally. 
%%If $\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']>0$, then there exist some tasks that have not been assigned to any server. 
%%In policy $P$, each idle server will be allocated to process an unassigned task from the job with the highest priority. Hence,
%%$\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']=\sum_{i: p_i\geq p} [\gamma_i - \zeta_i] - b \leq \sum_{i: p_i\geq p} \xi_i -b' \leq \sum_{i: p_i\geq p} \xi_i'$.
%%\end{proof}
%%
%%
%%\begin{lemma}\label{lem_non_prmp2_lem3}
%%Suppose that under policy $P$, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by adding a job with $b$ tasks and arrival time $a$ to the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that under policy $\pi$, $\bm{\xi}'$ is obtained by adding a job with $b$ tasks and arrival time $a$ to the system whose state is $\bm{\xi}$.
%%If
%%\begin{eqnarray}
%%\sum_{i: p_i\geq p} [\gamma_i- \zeta_i]\leq \sum_{i: p_i\geq p} \xi_i, ~\forall~p\geq 0,\nonumber
%%\end{eqnarray}
%%then
%%\begin{eqnarray}
%%\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i: p_i\geq p} \xi_i', ~\forall~p\geq 0.\nonumber\end{eqnarray}
%%\end{lemma}
%%
%%\begin{proof}
%%If $a\leq a_j$, then
%%$\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i: p_i\geq p} [\gamma_i - \zeta_i] + b\leq \sum_{i: p_i\geq p} \xi_i+b \leq \sum_{i: p_i\geq p} \xi_i'$.
%%
%%If $a>a_j$, then
%%$\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i: p_i\geq p} [\gamma_i - \zeta_i] \leq \sum_{i: p_i\geq p} \xi_i \leq \sum_{i: p_i\geq p} \xi_i'$.
%%\end{proof}
%%
%%The proof of Lemma \ref{lemG4_lem3} is quite similar with that of Lemma \ref{lemG4}, and hence is omitted. The only differences are (i) Lemma \ref{lem_non_prmp1} and Lemma \ref{lem_non_prmp2} in the proof of Lemma \ref{lemG4} should be replaced by Lemma \ref{lem_non_prmp1_lem3} and Lemma \ref{lem_non_prmp2_lem3}, respectively, and (ii) $\bm{\alpha}(t)$, $\bm{\delta}(t)$, and $\bm{\beta}(t)$ in the proof of Lemma \ref{lemG4} should be replaced by $\bm{\gamma}(t)$, $\bm{\zeta}(t)$, and $\bm{\xi}(t)$, respectively.
%%
%%
%%
%%
%%
%%
%%The second part of the sample-path ordering result is as follows:
%%
%%\begin{lemma}\label{lem_sample_path_ordering_lem3}
%%If Lemma \ref{lemG4_lem3} holds, then $\bm{u}_{\uparrow}(P)\leq \bm{c}_{\uparrow}(\pi)$ holds on sample path for all $\pi\in\Pi_{PL}$. 
%%\end{lemma}
%%
%%\begin{proof}
%%Let $w_i$ be the index of the job associated with $v_{(i)}(P)$, then job $w_j$ is the $j$-th job whose tasks are completed or under service in policy $P$. Similar with \eqref{eq_proof_3_thm3} in the proof of Lemma \ref{lem_sample_path_ordering_thm3}, we can obtain
%%\begin{align}
%%v_{w_j}(P) \leq \max_{i:a_i\leq v_{w_j}(P),p_i\geq p_{w_j} }c_{i}(\pi).
%%\end{align}
%%
%%Because job $w_j$ is the $j$-th job whose tasks are completed or under service, only the jobs $w_1,\ldots, w_{j-1}$ can be completed during $[0,v_{w_j}(P))$ in policy $P$.
%%In addition, each idle server is assigned to process a task from the job with the highest priority in  policy $P$. This tells us that job $w_j$ has the highest priority among all jobs in the queue at time $v_{w_j}(P)$ in policy $P$.
%%Therefore, if job $i$ satisfies $a_i\leq v_{w_j}(P)$ and $p_i\leq p_{w_j}$, then $i\in\{w_1,\ldots, w_j\}$. 
%%
%%
%%%We  prove Lemma \ref{lem_sample_path_ordering_lem3} by induction. 
%%Consider the sample paths of policy $P$ and policy $\pi$ in Lemma \ref{lemG4_lem3}. 
%%Recall that $U_i(P)$ is the earliest time that all tasks of job $i$ are either completed or under service in policy $P$, $v_i(P)$ is the realization of $U_i(P)$ on the sample path of policy $P$, and $v_{(i)}(P)$ is the $i$-th smallest component of $(v_{1}(P),\ldots,v_{n}(P))$. Let $w_i$ be the index of the job associated with $v_{(i)}(P)$.
%%
%%%\emph{Step 1: We first show that} 
%%%\begin{align}\label{eq_Condition_3_1_lem3}
%%%v_{w_1}(P) - d_{w_1} \leq c_{w_1}(\pi) - d_{w_1}.
%%%\end{align}
%%%%Let $y_1$ be the number of jobs that have arrived by time $v_{w_1}(P)$. 
%%%
%%%
%%%We prove \eqref{eq_Condition_3_1_lem3} by contradiction. Suppose that 
%%%\begin{align}\label{eq_Condition_3_11_lem3}
%%%v_{w_1}(P) > c_{w_1}(\pi),
%%%\end{align} 
%%%i.e., job $w_1$ is completed earlier than $v_{w_1}(P)$ in policy $\pi$. 
%%%
%%%Because job $w_1$ is the first job whose tasks are either completed or under service, no job is completed during $[0,v_{w_1}(P))$ in policy $P$. Because policy $P$ satisfies condition 2 of Thoerem \ref{lem3}, job $w_1$ has the earliest due time among all jobs in the queue at time $v_{w_1}(P)$ in policy $P$.  This tells us that job $w_1$ has the earliest due time among all jobs that have arrived during $[0,v_{w_1}(P))$.
%%%Hence, when job $w_1$ departs at time $c_{w_1}(\pi)$ in policy $\pi$, $d_i> d_{w_1}$ holds for all jobs in the queue. Therefore, the system state of policy $\pi$ satisfies  
%%%\begin{align}\label{eq_proof_0_lem3}
%%%\sum_{i:d_i\leq d_{w_1}}\xi_i(c_{w_1}(\pi)) =0.
%%%\end{align}
%%%Combining \eqref{eq_proof_0_lem3} and Lemma \ref{lemG4_lem3}, we can obtain
%%%%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(\pi)$ such that
%%%%Invoking Lemma \ref{lemG4}, we can obtain
%%%\begin{align}\label{eq_proof_1_lem3}
%%%\sum_{i:d_i\leq d_{w_1}} \gamma_i(c_{w_1}(\pi))\leq \sum_{i:d_i\leq d_{w_1}}  \zeta_i(c_{w_1}(\pi)).
%%%\end{align}
%%%By the definition of the system state of policy $P$, we have $\gamma_i(t)\geq \zeta_i(t)$ for all $i$ and $t$. This and \eqref{eq_proof_1_lem3} tells us that at time $c_{w_1}(\pi)$, the system state of policy $P$ satisfies
%%%\begin{align}\label{eq_proof_2_lem3}
%%%\!\!\gamma_{w_1}(c_{w_1}(\pi))= \zeta_{w_1}(c_{w_1}(\pi)).
%%%\end{align}
%%%Hence, in policy $P$ all tasks of job $w_1$ are either completed or under service at time $c_{w_1}(\pi)$. Combine this and \eqref{eq_Condition_3_11_lem3}, yields $$v_{w_1}(P)\leq c_{w_1}(\pi)<v_{w_1}(P),$$ which is a contradiction. Hence, $v_{w_1}(P) \leq c_{w_1}(\pi)$. By this, \eqref{eq_Condition_3_1_lem3} is proven.
%%
%%It is sufficient to show that for each $j=1,2,\ldots,n$,
%%\begin{align}\label{eq_Condition_3_12_lem3}
%%v_{w_j}(P)-d_{w_j} \leq \max_{i=1,2,\ldots,n }[c_{i}(\pi)-d_i].
%%\end{align}
%%We prove \eqref{eq_Condition_3_12_lem3} by contradiction. Suppose that 
%%\begin{align}\label{eq_proof_9_lem3}
%%v_{w_j}(P) > c_{i}(\pi)
%%\end{align}
%%holds for all $i$ satisfying $a_i\leq v_{w_j}(P)$ and $d_i\leq d_{w_j}$. That is, if job $i$ satisfies $d_i\leq d_{w_j}$ and $a_i\leq v_{w_j}(P)$, then job $i$ departs before time $v_{w_j}(P)$.
%%Hence, at time 
%%\begin{align}
%%\tau=\max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j}} c_{i}(\pi),\nonumber
%%\end{align} $d_i> d_{w_j}$ holds for all jobs in the queue in policy $\pi$. Therefore, the system state of policy $\pi$ satisfies  
%%\begin{align}
%%\sum_{i:d_i\leq d_{w_j}}\xi_i(\tau) =0.\nonumber
%%\end{align}
%%Combining this with Lemma \ref{lemG4_lem3}, we can obtain
%%%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(\pi)$ such that
%%%Invoking Lemma \ref{lemG4}, we can obtain
%%\begin{align}\label{eq_proof_1_lem3}
%%\sum_{i:d_i\leq d_{w_j}} [\gamma_i(\tau)-\zeta_i(\tau)]\leq 0.
%%\end{align}
%%By the definition of the system state of policy $P$, we have $\gamma_i(t)\geq \zeta_i(t)$ for all $i$ and $t$. This and \eqref{eq_proof_1_lem3} tells us that at time $t$, job $w_j$ in policy $P$ satisfies
%%\begin{align}
%%\gamma_{w_j}(\tau)= \zeta_{w_j}(\tau).\nonumber
%%\end{align}
%%That is, in policy $P$ all tasks of job $w_j$ are either completed or under service at time $\tau$. Hence, $v_{w_j}(P)\leq \tau$, which contradicts with  \eqref{eq_proof_9_lem3}. Therefore, $v_{w_j}(P) \leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi)$ and
%%\begin{align}
%%v_{w_j}(P)-d_{w_j} &\leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi)-d_{w_j} \nonumber\\
%%& \leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }[c_{i}(\pi)-d_{i}]\nonumber\\
%%&\leq \max_{i=1,2,\ldots,n }[c_{i}(\pi)-d_i].\nonumber
%%\end{align}
%%Hence, \eqref{eq_Condition_3_12_lem3} is obtained. This completes the proof.
%%\end{proof}
%%By considering all possible sample paths of these two policies, the stochastic ordering result in Thoerem \ref{lem3} follows.
%%\subsection{Proof of Corollary \ref{coro2}}
%%
%%In the proof of Corollary \ref{coro2}, we will need the following rearrangement inequality  : 
%%\begin{lemma} \cite[Theorem 6.F.14]{Marshall2011}\label{lem_rearrangement}
%%Consider two $n$-vectors $(x_1,\dots,x_n)$ and $(y_1,\ldots,y_n)$. If $x_i> x_j$ and $y_i<y_j$ for some indices $i$ and $j$ where $1\leq i<j\leq n$, then 
%%\begin{align}
%%&(x_1\!-\!y_1,\ldots,x_j\!-\!y_i,\ldots,x_i\!-\!y_j,\ldots,x_n\!-\!y_n)\nonumber\\
%%\prec& (x_1\!-\!y_1,\ldots,x_i\!-\!y_i,\ldots,x_j\!-\!y_j,\ldots,x_n\!-\!y_n).\nonumber
%%\end{align}
%%\end{lemma}
%%\ifreport
%%\begin{proof}[Proof of Corollary \ref{coro2}]
%%\else
%%\begin{proof}[of Corollary \ref{coro2}]
%%\fi
%%As in the proof of Lemma \ref{lem_sample_path_ordering_lem3}, let $w_i$ denote the index of the job associated with $v_{(i)}(P)$. 
%%
%%\emph{Step 1: We first show that  for all $j=1,\ldots,n$}
%%\begin{align}\label{eq_coro2_2}
%%v_{w_j}(P) \leq c_{(j)}(\pi).
%%\end{align}
%%
%%Suppose that $b_j$ tasks have been assigned to the servers in policy $P$ by time $c_{(j)}(\pi)$. Since each job has only one task, $j$ tasks are completed by time $c_{(j)}(\pi)$ in policy $\pi$.
%%Because policy $P$ is more work-efficient than policy $\pi$, it must hold that (i) at least $j$ unassigned task are allocated to the servers during $[0,c_{(j)}(\pi)]$  in policy $P$, i.e., $b_j\geq j$, or (ii) all the remaining tasks are under service at time $c_{(j)}(\pi)$  in policy $P$. Obviously, case (ii) belongs to case (i). Because each job has only one task, it follows that $v_{w_j}(P) \leq c_{(j)}(\pi)$  for all $j=1,\ldots,n$.
%%
%%%We prove Corollary \ref{coro2} by induction. 
%%
%%\emph{Step 2: We show that one of the following two cases is true:
%%\begin{itemize}
%%\item[1.] $v_{w_1}(P)\leq c_{w_1}(\pi)$, and $v_{w_{2}}(P)\leq c_{w_{2}}(\pi)$;
%%%\item[2.] $d_{w_j}\leq d_{w_{j+1}}$, $v_{w_j}(P)\leq c_{w_j}(\pi)$, and $v_{w_{j+1}}(P)\leq c_{w_{j+1}}(\pi)$.
%%\item[2.] $v_{w_1}(P)\leq c_{w_{2}}(\pi)$, $v_{w_{2}}(P)\leq c_{w_{1}}(\pi)$, $d_{w_1}\leq d_{w_{2}}$, and $c_{w_{1}}(\pi)>c_{w_{2}}(\pi)$.
%%\end{itemize}}
%%
%%In the proof of Lemma \ref{lem_sample_path_ordering_lem3}, it was shown that 
%%\begin{align}\label{eq_coro2_1}
%%v_{w_j}(P) \leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi).
%%\end{align}
%%
%%We first consider $j=1$. Because job $w_1$ is the first job whose tasks are either completed or under service, no job is completed during $[0,v_{w_1}(P))$ in policy $P$. Because policy $P$ satisfies condition 2 of Thoerem \ref{lem3}, job $w_1$ has the earliest due time among all jobs in the queue at time $v_{w_1}(P)$ in policy $P$. This tells us that if job $i$ satisfies $a_i\leq v_{w_1}(P)$ and $d_i\leq d_{w_1}$, then $i=w_1$. Hence,  \eqref{eq_coro2_1} implies 
%%$v_{w_1}(P) \leq c_{w_1}(\pi)$. 
%%
%%For $j=2$, because job $w_2$ is the second job whose tasks are either completed or under service, only  job $w_1$ can be completed during $[0,v_{w_2}(P))$ in policy $P$. Because policy $P$ satisfies condition 2 of Thoerem \ref{lem3}, job $w_2$ has the earliest due time among all jobs in the queue at time $v_{w_2}(P)$ in policy $P$. This tells us that if job $i$ satisfies $a_i\leq v_{w_2}(P)$ and $d_i\leq d_{w_2}$, then $i=w_1$ or $i=w_2$. 
%%
%%If $d_{w_1}> d_{w_2}$, then \eqref{eq_coro2_1} implies $v_{w_2}(P) \leq c_{w_2}(\pi)$. 
%%
%%If $d_{w_1}\leq d_{w_2}$, then \eqref{eq_coro2_1} implies $v_{w_2}(P) \leq \max[c_{w_1}(\pi), c_{w_2}(\pi)]$. We first consider two sub-cases: If $c_{w_1}(\pi)\leq c_{w_2}(\pi)$, then $v_{w_2}(P) \leq c_{w_2}(\pi)$. 
%%If $c_{w_1}(\pi)> c_{w_2}(\pi)$, by \eqref{eq_coro2_2}, we can obtain $v_{w_1}(P) \leq c_{w_2}(\pi)$ and $v_{w_2}(P)\leq c_{w_1}(\pi)$.
%%
%%By summarizing these cases, the claim of \emph{Step 2} follows. 
%%
%%\emph{Step 3: We show that}
%%\begin{align}\label{eq_coro2_3}
%%\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}.
%%\end{align} 
%%
%%We carry out the following operation: 
%%If case 2 of \emph{Step 2} holds, we interchange the completion times of job $w_1$ and job $w_2$. 
%%%By Lemma \ref{lem_rearrangement}, we can obtain
%%%\begin{align}
%%%&(c_{w_2}(\pi)\!-\!d_{w_1},c_{w_1}(\pi)\!-\!d_{w_2},c_{w_3}(\pi)\!-\!d_{w_3},\ldots,c_{w_n}(\pi)\!-\!d_{w_n})\nonumber\\
%%%\prec& (c_{w_1}(\pi)\!-\!d_{w_1},c_{w_2}(\pi)\!-\!d_{w_2},c_{w_3}(\pi)\!-\!d_{w_3},\ldots,c_{w_n}(\pi)\!-\!d_{w_n}).\nonumber
%%%\end{align}
%%If case 1 of \emph{Step 2} holds, there is no interchange. 
%%Let $\bm{c}^{0} (\pi)=\bm{c}(\pi)$ and $\bm{c}^{1} (\pi)$, respectively, denote the completion time vectors of the $n$ jobs before and after this operation. By Lemma \ref{lem_rearrangement}, we can get 
%%\begin{align}
%%\bm{c}^{1} (\pi)-\bm{d}\prec \bm{c}^{0} (\pi)-\bm{d}.\nonumber
%%\end{align}
%%In addition, it holds that $v_{w_1}(P)\leq c^{1}_{w_1}(\pi)$, and $v_{w_{2}}(P)\leq c^{1}_{w_{2}}(\pi)$.	
%%We repeating this operation $n-1$ times. More specifically, in the $l$-th operation, for each $i=1,\ldots,l$ if $d_{w_i}\leq d_{w_{l+1}}$ and $c^{l-1}_{w_{i}}(\pi)>c^{l-1}_{w_{l+1}}(\pi)$, we interchange job $w_i$ and job $w_{l+1}$. Let $\bm{c}^{l} (\pi)$ denote the completion time vectors of the $n$ jobs after the $l$-th operation.
%%Using \eqref{eq_coro2_2}, \eqref{eq_coro2_1}, and condition 2 of Thoerem \ref{lem3}, we can obtain 
%%\begin{align}
%%&\bm{c}^{n-1} (\pi)-\bm{d} \prec \ldots \prec \bm{c}^{1} (\pi)-\bm{d} \prec \bm{c}^{0} (\pi)-\bm{d}, \nonumber\\
%%&\bm{u}(P)\leq \bm{c}^{n-1}(\pi).\nonumber
%%\end{align}
%%Hence,
%%\begin{align}
%%\bm{u}(P)-\bm{d}\leq \bm{c}^{n-1}(\pi)-\bm{d}\prec \bm{c} (\pi)-\bm{d}.\nonumber
%%\end{align} 
%%By this, \eqref{eq_coro2_3} follows. According to Theorem 3.A.8 of \cite{Marshall2011}, $f(\bm{u}(P)-\bm{d}) \leq f(\bm{c} (\pi)-\bm{d})$ holds for all $f\in\mathcal{D}_{\text{Sch}}$. This completes the proof.
%%\end{proof}

==> appendices_5.tex <==
% !TEX root = ./replication.tex

\section{Proofs of Thoerem~4 and Corollary 6} \label{app4}
\subsection{Proof of Thoerem~\ref{thm4}} \label{sec_app_4_1}
We prove Thoerem~\ref{thm4} by using Lemma \ref{lem2}, where the policy space $\Pi$ is replaced by $\Pi_{\text{non-prmp}}$ because preemption is not allowed. The proof steps are as follows:

{\bf Construction of Policy $P'$:}
We construct an {infeasible} policy $P'$. Similar with policy EDD-R, when all servers are idle in policy $P'$, a task from the job with the earliest due time is replicated on all $m$ servers. When a copy of this task is completed, the remaining $m-1$ replicated copies of this task are cancelled. The difference between policy EDD-R and policy $P'$ is that \emph{the completed tasks of policy $P'$ are relabelled such that each completed task is from the job with the earliest due time}. (This relabeling operation might be infeasible in the following scenario: If a job with an earlier due time arrives, the servers cannot be reassigned to this incoming job because preemption is not allowed. However, the next completed task is relabelled to be from this incoming job which has the earliest due time.) By this, policy $P'$ is constructed.

Next, we prove the conditions of Lemma \ref{lem2} one by one.

\textbf{Condition 1:} \emph{Policy $P'$ is more {work-efficient} than any policy $\pi\in\Pi_{\text{non-prmp}}$}. Condition 1 can be proven by using the same proof arguments in Appendix \ref{sec_app_thm2_1}.

\textbf{Condition 2:} \emph{Each completed task of policy $P'$ belongs to the job with the earliest due time}. Condition 2 directly follows from the construction of policy $P'$.

\textbf{Condition 3:} \emph{It holds that} 
\begin{align}\label{eq_condition3_thm4}
[\bm{U}_{}(\text{EDD-R})|\mathcal{I}] \leq_{\text{st}} [\bm{C}_{}(P')|\mathcal{I}].
\end{align}

We prove condition 3 by using the \emph{sample-path ordering} technique. The system state $\bm{\xi}$ of policy $P'$ is the same as that in \emph{Definition \ref{def_state_P_thm3}}. The system state $(\bm{\gamma},\bm{\zeta})$ of policy EDD-R is the same as that in \emph{Definition \ref{def_state_thm3}}. 
In policy EDD-R, all servers are simultaneously assigned to process $m$ replicated copies of the same task. Hence, $\bm{\zeta}$ satisfies
\begin{align}
\zeta_i\in\{0,1\},~\sum_{i=1}^n \zeta_i\leq1.
\end{align}
We can prove that Lemmas \ref{lemG4_thm3}-\ref{lem_non_prmp2_thm3} hold for policy EDD-R. 
Using Lemma \ref{lemG4_thm3}, condition 3 can be proven by using the same proof arguments in Appendix \ref{sec_app_3_1}, where policy EDD-NR should be replaced by policy EDD-R.

After establishing conditions 1-3 of Lemma \ref{lem2} for policy EDD-R,  we can use Lemma \ref{lem2} to prove Theorem \ref{thm4}. This completes the proof.

\subsection{Proof of Corollary~\ref{coro4_2}}  
If $d_1\leq\ldots\leq d_n$, then each completed task of policy EDD-R belongs to the job with the earliest due time. Therefore, policy EDD-R is identical with policy $P'$ constructed in Appendix \ref{sec_app_4_1}. Then, Corollary \ref{coro4_2} follows from Lemma \ref{lem2}. 

\subsection{Proof of Corollary~\ref{coro4_1}} \label{sec_app_4_2} 
Because conditions 1-3 of Lemma \ref{lem2} have been established in Appendix \ref{sec_app_4_1},  Corollary~\ref{coro4_1} directly follows from Corollary \ref{coro2}.

==> appendices_6.tex <==
% !TEX root = ./replication.tex

\section{Proof of Thoerem~5} \label{app5}

\subsection{Proof of \eqref{eq_delaygap1_thm5} in Thoerem~5}
We prove \eqref{eq_delaygap1_thm5} in Thoerem~\ref{thm5} by using Lemma \ref{lem3}. In particular, we will use the \emph{sample-path ordering} technique to prove condition \eqref{eq_lem3_1} of Lemma \ref{lem3}.
We first define the system states of policy PL-NR and any policy $\pi\in\Pi_{PL}$, where $PL=(p_1,\ldots,p_n)$ denote a static priority list.

\begin{definition}\label{def_state_P_thm5}
The system state of policy $\pi\in\Pi_{PL}$ is specified by a pair of $n$-dimensional vectors $\bm{\xi}=(\xi_1,\ldots,\xi_n)$ and $\bm{\kappa}=(\kappa_1,\ldots,\kappa_n)$ with non-negative components. At any time, if job $i$ exists in the system, $\xi_i$ is the number of remaining tasks of job $i$ and $\kappa_i$ out of these $\xi_i$ tasks are under service on some servers; if job $i$ has not arrived at the system or has departed from the system, $\xi_i=\kappa_i=0$. Hence, 
\begin{align}%\label{eq_def_state_P_thm5}
\kappa_i  \leq \xi_i \leq k_{i},~\sum_{i=1}^n \kappa_i \leq m. \nonumber
\end{align}
\end{definition}

\begin{definition}\label{def_state_thm5}
The system state of policy PL-NR is specified by a pair of $n$-dimensional vectors $\bm{\gamma}=(\gamma_1,\ldots,\gamma_n)$ and $\bm{\zeta}=(\zeta_1,\ldots,\zeta_n)$ with non-negative components. 
At any time, if job $i$ exists in the system, then $\gamma_i$ is the number of remaining tasks of job $i$ and $\zeta_i$ out of these $\gamma_i$ tasks are under service on some servers; if job $i$ has not arrived at the system or has departed from the system, then $\gamma_i=\zeta_i=0$.
Hence, 
\begin{align}%\label{eq_def_state_thm5}
\zeta_i  \leq \gamma_i \leq k_{i},~\sum_{i=1}^n \zeta_i \leq m. \nonumber
\end{align}
\end{definition}

Let $\{\bm{\xi}(t),\bm{\kappa}(t),t\geq0\}$ be the state process of policy $\pi$, and $\{\bm{\gamma}(t),\bm{\zeta}(t),t\geq0\}$ be the state process of PL-NR, which are assumed to be right-continuous. 
The sample-path ordering result is stated in the following lemma:
 
 
\begin{lemma}\label{lemG4_thm5}
Suppose that $\bm{\xi}(0^-)=\bm{\kappa}(0^-)=\bm{\gamma}(0^-)=\bm{\zeta}(0^-)=\bm{0}$ and the job parameters $\mathcal{I}$ are given. For any sample path of policy PL-NR, there exists a sample path of policy $\pi$ with the same probability density such that
\begin{eqnarray}\label{eq_lemG4_thm5}
\sum_{i:p_i\geq p} [\gamma_i(t) - \zeta_i(t)]\leq \sum_{i:p_i\geq p} [\xi_i(t)-\kappa_i(t)], 
\end{eqnarray}
holds for all $t\geq0$ and $p = 1,2,\ldots,n$.
\end{lemma}

The following two lemmas are needed to prove Lemma \ref{lemG4_thm5}:


\begin{lemma}\label{lem_non_prmp1_thm5}
Suppose that, under policy PL-NR, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by completing a task on one server in the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that, under policy $\pi$, $\{\bm{\xi}',\bm{\kappa}'\}$ is obtained by completing a task on one server in the system whose state is $\{\bm{\xi},\bm{\kappa}\}$. If
\begin{eqnarray}
\sum_{i:p_i\geq p} [\gamma_i - \zeta_i]\leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i], ~\forall~p = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40_thm5}
\sum_{i:p_i\geq p} [\gamma_i'- \zeta_i']\leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i'], ~\forall~p = 1,2,\ldots,n.\end{eqnarray}
\end{lemma}

\begin{proof}
If $\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']=0$, then the inequality \eqref{eq_non_prmp_40_thm5} follows naturally. 
If $\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']>0$, then there exist some tasks that have not been assigned to any server. 
In both policy PL-NR and policy $\pi$, a server that has just completed a task will be allocated to process an unassigned task from the job with the highest priority among all jobs in the queue. Hence,
$\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']=\sum_{i:p_i\geq p} [\gamma_i - \zeta_i] - 1 \leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i] -1 \leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i']$.
\end{proof}


\begin{lemma}\label{lem_non_prmp2_thm5}
Suppose that, under policy PL-NR, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by adding a job with $b$ tasks and priority $d$ to the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that, under policy $\pi$, $\{\bm{\xi}',\bm{\kappa}'\}$ is obtained by adding a job with $b$ tasks and priority $d$ to the system whose state is $\{\bm{\xi},\bm{\kappa}\}$.
If
\begin{eqnarray}
\sum_{i:p_i\geq p} [\gamma_i- \zeta_i]\leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i], ~\forall~p = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i'], ~\forall~p = 1,2,\ldots,n.\nonumber\end{eqnarray}
\end{lemma}

\begin{proof}
If $d\geq p$, then
$\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i:p_i\geq p} [\gamma_i - \zeta_i] + b\leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i]+b \leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i']$.

If $d<p$, then
$\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i:p_i\geq p} [\gamma_i - \zeta_i] \leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i] \leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i']$.
\end{proof}

Now we are ready to prove Lemma \ref{lemG4_thm5}.
\ifreport
\begin{proof}[Proof of Lemma \ref{lemG4_thm5}]
\else
\begin{proof}[of Lemma \ref{lemG4_thm5}]
\fi
Consider any period $[\tau,\nu)$ of policy PL-NR, during which there are at least $m$ tasks such that all $m$ servers are busy. We prove \eqref{eq_lemG4_thm5} for $t\in[\tau,\nu)$ by considering two cases:

\emph{Case 1: At time $t=\tau$, policy PL-NR has $m$ tasks and the service of these tasks has just started.} Consider the system states of both policies at time $\tau$. The system state of policy PL-NR satisfies 
\begin{align}\label{proof_lemG4_1_thm5}
\sum_{i=1}^n \gamma_i(\tau)= m, ~\bm{\gamma}(\tau)=\bm{\zeta}(\tau).
\end{align}
In policy $P'$, there is no task in the system at time $\tau^-$ such that 
\begin{align}\label{proof_lemG4_5_thm5}
\bm{\xi}(\tau^-)=\bm{0}. 
\end{align}
Consider the evolutions of both policies during $[\tau,\nu)$. 
In policy $P'$, all servers are busy if there is at least one task. On the other hand, in policy EDD-NR, there is no task replication and all servers are busy if there are no less than $m$ tasks. 
By \eqref{proof_lemG4_1_thm5} and \eqref{proof_lemG4_5_thm5}, it holds that for $t=\tau$
\begin{align}\label{proof_lemG4_4_thm5}
\sum_{i=1}^n \gamma_i(t)= \sum_{i=1}^n\xi_i(t) +m\geq m+1.
\end{align}
Therefore, the servers are all busy in policies $P'$ and policy EDD-NR at time $\tau$. By induction over time, we can show that for any sample path of policy $P'$, there is a sample path of policy EDD-NR with the same probability density such that \eqref{proof_lemG4_4_thm5} holds for all $t\in[\tau,\nu)$ and the task arrival times and task completion times of the two policies are exactly the same  during $[\tau,\nu)$. Using Lemma \ref{lem_non_prmp1_thm5}, Lemma \ref{lem_non_prmp2_thm5}, and the initial states at time $\tau^-$, we can prove that \eqref{eq_lemG4_thm5} holds for all $t\in[\tau,\nu)$ on these two sample paths.

\emph{Case 2: At time $t=\tau^-$, policy EDD-NR has less than $m$ tasks or the service of these tasks started before time $\tau^-$}. In both \emph{Case 1} and \emph{Case 2}, the sample path evolutions of policy $P'$ are the same. On the other hand, in policy EDD-NR, the tasks are completed earlier in \emph{Case 2} than in \emph{Case 1}. Therefore, \eqref{eq_lemG4_thm5}  also holds in \emph{Case 2} for $t\in[\tau,\nu)$.

%Note that the case that policy EDD-NR has more than $m$ tasks at time $\tau^-$ will not happen. This will be clear 
Let $[\tau_1,\nu_1)$ be the next busy period of policy $P'$ with $\nu<\tau_1$. Then, $[\nu,\tau_1)$ is an idle period of policy $P'$. We now prove \eqref{eq_lemG4_thm5} during the idle period $[\nu,\tau_1)$. 
Because all servers are idle during $[\nu,\tau_1)$ in policy $P'$, it follows that 
\begin{align}\label{proof_lemG4_2_thm5}
\bm{\xi}(t)=\bm{0},~t\in[\nu,\tau_1).
\end{align}
Hence, there is no task arrival during $[\nu,\tau_1)$; otherwise, \eqref{proof_lemG4_2_thm5} cannot be true.
On the other hand, at time $\nu$ there are no more than $m$ tasks in policy EDD-NR such that 
\begin{align}
\bm{\gamma}(\nu)=\bm{\zeta}(\nu).\nonumber
\end{align}
Because there is no task arrival during $[\nu,\tau_1)$, policy EDD-NR satisfies
\begin{align}\label{proof_lemG4_3_thm5}
\bm{\gamma}(t)=\bm{\zeta}(t),~t\in[\nu,\tau_1).
\end{align}
By \eqref{proof_lemG4_2_thm5} and \eqref{proof_lemG4_3_thm5}, \eqref{eq_lemG4_thm5} holds during $[\nu,\tau_1)$.
Further, from \eqref{proof_lemG4_3_thm5}, we can obtain
\begin{align}
\sum_{i=1}^n \gamma_i(\tau_1^-)=\sum_{i=1}^n \zeta_i(\tau_1^-)\leq m,
\end{align}
such that there are no more than $m$ tasks at time $t=\tau_1^-$ in policy EDD-NR. Hence, either \emph{Case 1} or \emph{Case 2} is satisfied at time $t=\tau_1^-$. Then, we can use the above arguments to prove that  \eqref{eq_lemG4_thm5} holds during the next busy period $[\tau_1,\nu_1)$ of policy $P'$.


Finally, by taking an induction over the busy and idle periods of policy $P'$,  Lemma \ref{lemG4_thm5} is proven.
\end{proof}



After establishing conditions 1-3 of Lemma \ref{lem2} for policy EDD-R,  we can use Lemma \ref{lem2} to prove Theorem \ref{thm4}. This completes the proof.

\subsection{Proof of Corollary~\ref{coro4_2}}  
If $d_1\leq\ldots\leq d_n$, then each completed task of policy EDD-R belongs to the job with the earliest due time. Therefore, policy EDD-R is identical with policy $\pi$ constructed in Appendix \ref{sec_app_4_1}. Then, Corollary \ref{coro4_2} follows from Lemma \ref{lem2}. 

\subsection{Proof of Corollary~\ref{coro4_1}} \label{sec_app_4_2} 
Because conditions 1-3 of Lemma \ref{lem2} have been established in Appendix \ref{sec_app_4_1},  Corollary~\ref{coro4_1} directly follows from Corollary \ref{coro2}.

==> sufficient_conditions.tex <==
% !TEX root = ./replication.tex

%\section{Sufficient Conditions for Delay Optimality and Near-Optimality}


\section{Sufficient Conditions for Near Delay Optimality}\label{sec_sufficient}
%\section{Proof Structure}
%The existing proof techniques for the delay optimality or near optimality of task replication policies are combinatorial and  difficult to understand. There is a lack of unify framework to unify different proof techniques.  As an attempt to alleviate this difficulty, 

%Existing delay optimality and near delay optimality analyses of task replications \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013,ShengboInfocom,Sun2015} focused on the average delay ${D}_{\text{avg}}(\cdot)$, and their proof techniques vary from case to case. 
%There is a lack of unified treatment for minimizing different delay metrics in various system settings. 
In this section, we establish a unified framework for minimizing several classes of delay metrics in various system settings. In particular, sufficient conditions are proposed for proving that a scheduling policy is near delay-optimal, %These sufficient conditions do not need to specify the queueing model or service time distribution, and hence provide a unified treatment for various system settings. 
%In addition, 
%These sufficient conditions can handle not only the average delay ${D}_{\text{avg}}(\cdot)$, but also more general delay metric functions in $\mathcal{D}_{\text{sym}}$, $\mathcal{D}_{\text{Sch-1}}$, and $\mathcal{D}_{\text{Sch-2}}$. 
% for various system settings.
%These sufficient conditions
which will be used to establish our main results in later sections. These sufficient conditions are proven by using stochastic ordering and majorization.
%A \textbf{sample-path ordering} technique is developed to prove 
 %Note that the bounds that we will describe are by no means the tightest that are available from the sample-path ordering technique. In particular, different bounds can be obtained from different forms of sample-path ordering, which will be studied in our future work.
%for centralized queue systems in Section \ref{sec_analysis}, and for distributed queue systems in Section \ref{sec_distributed}.
% for distribued delay metrics and system settings.

%which provide a unified framework in minimizing a number of delay metrics. These sufficient conditions do not depend on a specific system setting, independent, The existing proof techniques for the delay optimality or near optimality results of task replication policies  
%are combinatorial and 
%vary from case to case, 
%which makes them difficult to understand, 
%which do not provide a unified treatment for different system settings.
% and do not provide a unified treatment. 
% combinatorial and  difficult to understand. There is a lack of unify framework to unify different proof techniques.  
%As an attempt to alleviate this difficulty, 


%These sufficient conditions will be used in later sections to %outline the key proof steps of 
%which will be used later sections to prove near delay optimality results in various system settings. 


%We will see that the sufficient conditions for different delay metrics can be expressed in similar forms to provide a unified treatment for different delay metrics, but their proof techniques are different. 
%

%Moreover, in order to compare the task completion times among different scheduling policies, we develop a \emph{sample-path ordering} technique, which enables us to  prove near delay optimality results in the form of \eqref{eq_nearoptimal}. 
%The results of this section are proven in Appendix \ref{app0}.

%When using these sufficient conditions, one key difficulty is to prove that a scheduling policy is near-optimal in terms of \eqref{eq_nearoptimal}. To that end, we develop a novel technique called \emph{sample-path ordering}, which can effectively characterize the delay gap from the optimum. 
%\subsection{} 


%In this section, we propose novel sufficient conditions for proving that a scheduling policy is  delay-optimal or near-optimal. These sufficient conditions reveal the key ideas in delay optimality analysis of task replications and can greatly simplify the corresponding proof arguments.  The proofs of these sufficient conditions are provided in Appendix \ref{app0}.

% showing the existence of a low-complexity policy that is within a finite gap from the optimum delay.
%There is a lack of uniform methodology for bounding the sub-optimality gap from the optimum delay performance.

%Their usage will be illustrated in later sections when studying task replications across heterogeneous servers.

%In this section, we present a general analysis framework of
%redundant executions which serves two purposes: (i) to provide
%sufficient conditions for identifying scheduling policies that
%are delay-optimal or near-optimal, and (ii) to simplify and
%unify the proof techniques for establishing delay optimalityalleviate
%and near-optimality. These analysis tools will be used later tocumbersome
%study redundancy scheduling across heterogeneous servers.

 
%Define $\bm{s}=(s_{1},\ldots, s_{k_{\text{sum}}})$ as the sequence of task arrival times of the system, and $\bm{T}(\pi)=(T_{1}(\pi),\ldots, T_{k_{\text{sum}}}(\pi))$ as the sequence of task completion times of the system. The components of $\bm{s}$ and $\bm{T}(\pi)$ are arranged in the increasing order such that $\bm{s} =\bm{s}_{\uparrow}$ and $\bm{T}(\pi)=\bm{T}_{\uparrow}(\pi)$.~Then, $\bm{s}$ is uniquely determined by $\mathcal{I}$, while $\bm{T}(\pi)$ is determined by $\mathcal{I}$, the scheduling policy $\pi$, and random task service times.
\subsection{Work-Efficiency Ordering}

In traditional queueing systems without task replications, the service delay is largely governed by the following work conservation law (or its generalizations): At any time, the expected total amount of time for completing the jobs in the queue is invariant among all work-conserving policies \cite{Leonard_Kleinrock_book,Gittins:11}. However, this work conservation law does not hold in queueing system with task replications.
%, because each task has multiple replication modes. 
In particular, each task has multiple replication modes (i.e., it can be replicated on different numbers of servers and at different time instants), which require different amounts of service time. In order to minimize delay, the scheduler needs to choose efficient replication modes to execute the tasks. Motivated by this, we define a work-efficiency ordering to compare the efficiency of task executions in different task replication policies, where the job indices of the tasks are not concerned. 
%One illustration of this is provided in Fig. \ref{Work_Efficiency_Ordering}.



% Consider two non-preemptive feasible policies $\pi_1,\pi_2\in\Pi$. Suppose that the 


% in policy $\pi_1$ the tasks are executed in a more efficient replication mode than in policy $\pi_2$, then one would expect the . If , then in policy $\pi_1$ no fewer than $b$ tasks start execution during $[\tau,\nu]$, which may complete execution after time $\nu$ because 







%Define $\bm{s}=(s_{1},\ldots, s_{k_{\text{sum}}})$ as the sequence of task arrival times of the system, and $\bm{T}(\pi)=(T_{1}(\pi),\ldots,$ $ T_{k_{\text{sum}}}(\pi))$ as the sequence of task completion times of the system. The components of $\bm{s}$ and $\bm{T}(\pi)$ are arranged in the increasing order such that $\bm{s} =\bm{s}_{\uparrow}$ and $\bm{T}(\pi)=\bm{T}_{\uparrow}(\pi)$.~Then, $\bm{s}$ is uniquely determined by $\mathcal{I}$, while $\bm{T}(\pi)$ is determined by $\mathcal{I}$, the scheduling policy $\pi$, and random task service times.

%Let $k_{\text{sum}}=\sum_{i=1}^nk_i$ denote the total number of tasks, $\bm{t}(\pi)=(t_{1}(\pi),\ldots, t_{k_{\text{sum}}}(\pi))$ denote the realizations of task completion times on a sample path of policy $\pi$. The components of $\bm{t}(\pi)$ are arranged in the increasing order such that $\bm{t} (\pi)=\bm{t}_{\uparrow}(\pi)$.

%A relationship between two policies $\pi_1$ and $\pi_2$ is said to \textbf{hold on sample path}, if there is a measure preserving one-to-one correspondence between the sample paths of policies $\pi_1$ and $\pi_2$, such that  the relationship holds between each pair of corresponding sample paths of policies $\pi_1$ and $\pi_2$.

%We define a \emph{work efficiency order}:

%For any time interval $[\tau,\nu]$ and policy $\pi$, let $n_{{s}}^{\pi}(\tau,\nu)$ denote the number of tasks that start execution during $[\tau,\nu]$, and $n_{sc}^{\pi}(\tau,\nu)$ denote the number of tasks that start and complete execution during $[\tau,\nu]$. 

A relationship between policy $\pi_1$ and policy $\pi_2$ is said to \textbf{hold in stochastic ordering}, if for each sample path of policy $\pi_1$ there is a corresponding sample path of policy $\pi_2$, such that (i) these two sample paths of policy $\pi_1$ and policy $\pi_2$ have the same probability density, and (ii) the relationship holds between these two sample paths of policy $\pi_1$ and policy $\pi_2$.

\begin{definition} \label{def_order} \textbf{Work-Efficiency Ordering:}
A work-conserving policy $\pi_1\in\Pi$ is said to be \textbf{more work-efficient} than policy $\pi_2\in\Pi$, if 
the following relationship between policy $\pi_1$ and policy $\pi_2$ holds in stochastic ordering: For each task $j$ executed in  policy $\pi_2$, if 
\begin{itemize}
\item[1.] Task $j$ starts execution at time $\tau$ and completes execution at time $\nu$ on the sample path of policy $\pi_2$ where $\nu\geq\tau$, 
\item[2.] There exist unassigned tasks in the queue during $[\tau,\nu]$ on the corresponding sample path of policy $\pi_1$, 
\end{itemize}
then  on the sample path of policy $\pi_1$ there exists one corresponding task $j'$ which starts execution during $[\tau,\nu]$. 
\end{definition}

An illustration of the work-efficiency ordering is provided in Fig. \ref{Work_Efficiency_Ordering}. Informally speaking, policy $\pi_1$ is said to be more work-efficient than policy $\pi_2$, if the tasks are executed faster in policy $\pi_1$ than in policy $\pi_2$. In particular, if the service duration of task $j$ is $[\tau,\nu]$ on the sample path of policy $\pi_2$, then there  exists one task $j'$ whose service time is shorter than $\nu-\tau$ on the corresponding sample path of policy $\pi_1$. Because the task service of policy $\pi_1$ and policy $\pi_2$ is asynchronized, the executions of task $j$ and task $j'$ may start at different time instants. Hence, task $j'$ may start execution during $[\tau,\nu]$, and complete execution either before or after time $\nu$. We note that work-efficiency ordering is defined on task-level, which is not related to the service priority of different jobs. For this reason, the job indices of task $j$ and task $j'$ are not specified in the definition.

% speed  determined by the job indices of task $j$ and task $j'$ are not specified because they do not affect the efficiency of policy $\pi_1$ and policy $\pi_2$.


% the task service of policy $\pi_1$ and policy $\pi_2$ is asynchronized

%If on the sample path of policy $\pi_2$, one server starts to process a task at time $\tau$ and completes this task at time $\nu$ ($\tau\leq\nu$), then  on the sample path of policy $\pi_1$ there exists a time $t\in[\tau,\nu]$ such that one of the following three cases holds:  (i) the same server starts to process a corresponding task at time $t$ (as illustrated in Fig. \ref{Work_Efficiency_Ordering}), (ii) all the remaining tasks are under service at time $t$, or (iii) the queue is empty at time $t$.


%for any time interval $[\tau,\nu]$ if $b$ tasks start execution and also complete execution during $[\tau,\nu]$ in policy $\pi_2$, then one would expect that in policy $\pi_1$ no fewer than $b$ tasks start execution during $[\tau,\nu]$ (unless there are not enough tasks to execute in policy $\pi_1$); however, these tasks may complete execution after time $\nu$ in policy $\pi_1$, because the task service of policy $\pi_1$ and policy $\pi_2$ is asynchronized. 
%By this, the work-efficiency ordering can be defined as follows:


%This definition can be understood as follows: If each task is executed in a more efficient mode in policy $\pi_1$ than policy $\pi_2$, then the service duration of the task is shorter in policy $\pi_1$ than policy $\pi_2$. Because policy $\pi_1$ and policy $\pi_2$ are asynchronized, if $b$ tasks start and complete execution during $[\tau,\nu]$ on the sample path of policy $\pi_2$, than at least $b$ 


% $\pi_1\in\Pi$ is said to be \textbf{more work-efficient} than policy $\pi_2\in\Pi$


% $[\tau,\nu]$ and all servers are busy execution during $[\tau,\nu]$
%
%
%, if all servers are busy during $[\tau,\nu]$  on the sample path of policy $\pi_1$, then
%\begin{align}
%n_{{s}}^{\pi_1}(\tau,\nu)\geq_{\text{st}}  n_{sc}^{\pi_2}(\tau,\nu),
%\end{align}
%where $n_{{s}}^{\pi_1}(\tau,\nu)$ is the number of tasks that start execution during $[\tau,\nu]$  on the sample path of policy $\pi_1$, and $n_{sc}^{\pi_2}(\tau,\nu)$ is the number of tasks that start and complete execution during $[\tau,\nu]$  on the corresponding sample path of policy $\pi_2$.
% all servers are busy and $b$ tasks start execution in a time interval on the sample path of policy $\pi_1$, then no more than $b$ tasks start and complete execution in the same time interval on the sample path of policy $\pi_2$.
%$b$ tasks start and complete execution during $[\tau,\nu]$ on the sample path of policy $\pi_2$, then on the sample path of policy $\pi_1$, it holds that either $b$ tasks start execution during $[\tau,\nu]$ or all the remaining tasks are under service at some time $t\in[\tau,\nu]$.

%for all time interval $[\tau,\nu]\subseteq[0,\infty)$ and job parameters $\mathcal{I}$
%\begin{align}
%[N_{{a}}^{\pi_1}(\tau,\nu)| \mathcal{I}]\geq_{\text{st}}  [N_{ac}^{\pi_2}(\tau,\nu)| \mathcal{I}].
%\end{align}
%the following relationship holds on sample path: 
%\begin{itemize}
%\item[1.] $\bm{t}(\pi_1)\leq\bm{t}(\pi_2)$ holds on sample path.
%
%\item[2.] 
%For all $j=1,\ldots,n$ and $t\in[a_j,a_{j+1})$, 

%If on the sample path of policy $\pi_2$, one server starts to process a task at time $\tau$ and completes this task at time $\nu$ ($\tau\leq\nu$), then  on the sample path of policy $\pi_1$ there exists a time $t\in[\tau,\nu]$ such that one of the following three cases holds:  (i) the same server starts to process a corresponding task at time $t$ (as illustrated in Fig. \ref{Work_Efficiency_Ordering}), (ii) all the remaining tasks are under service at time $t$, or (iii) the queue is empty at time $t$.

\begin{figure}
\centering 
\includegraphics[width=0.4\textwidth]{Figures/work_efficiency_ordering} \caption{Illustration of work-efficiency ordering, where the service duration of a task is indicated by a rectangle. If on the sample path of policy $\pi_2$, task $j$ starts execution at time $\tau$ and completes execution at time $\nu$, then on the sample path of policy $\pi_1$ one corresponding task $j'$ starts execution at some time $t\in[\tau,\nu]$. The job indices of task $j$ and task $j'$ are not specified because they do not affect the efficiency of policy $\pi_1$ and policy $\pi_2$.}
% work--efficiency ordering holds for any priorities of the jobs.
\label{Work_Efficiency_Ordering} 
\end{figure} 
%or (ii') {one server is idle at time $\tau$}.\footnote{Note that the difference between these two definitions are in condition (ii) and condition (ii').}


%$b$ unassigned tasks are allocated to the servers and completed by the servers during $[a_j,t]$ on the sample path of policy $\pi_2$, then on the corresponding sample path of policy $\pi_1$ one of the following cases holds: (i) no fewer than $b$ unassigned tasks are allocated to the servers  during $[a_j,t]$, (ii) all the remaining tasks are under service at time $t$, or (iii) the queue is empty at time $t$.
%\end{itemize}
%in policy $\pi_2$ the system starts to process a task at time $\tau$ and completes the task at time $\nu$ ($\tau\leq\nu$), then in policy $\pi_1$ it holds that (i) a task is completed at some time during $[\tau,\nu]$, or (ii) {the queue is empty at time $\tau$}.
%for any sample path of policy $\pi_2$, there exists a sample path of policy $\pi_1$ with the same probability density such that $\bm{t}(\pi_1)\leq\bm{t}(\pi_2)$.
%Policy $\pi_1$ is said to be \emph{weakly more work-efficient} than policy $\pi_2$, if the following relationship holds on sample path: If in policy $\pi_2$ the system starts to process a task at time $\tau$ and completes the task at time $\nu$ ($\tau\leq\nu$), then in policy $\pi_1$ it holds that (i) a task is completed at some time during $[\tau,\nu]$, or (ii') {one server is idle at time $\tau$}.\footnote{Note that the difference between these two definitions are in condition (ii) and condition (ii').}


%The proof of the following lemma is straightforward and thus omitted: 
%\begin{theorem}\label{lemma_work_efficiency}
%If policy $\pi_1$ is {more work-efficient} than policy $\pi_2$, then
%\begin{itemize}
%\itemsep0em 
%\item[1.] policy $\pi_1$ is {weakly more work-efficient} than policy $\pi_2$;
%\item[2.] $\bm{t}(\pi_1)\leq\bm{t}(\pi_2)$ holds on sample path.
%\end{itemize} 
%\end{lemma}


%
\subsection{Sample-Path Ordering and Sufficient Conditions for Near Optimality}
In the special case that each job has one task, sufficient conditions are provided in \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013} for minimizing 
%if policy $P\in\Pi$ is more {work-efficient} than all $\pi\in\Pi$, then policy $P$ minimizes 
the average delay ${D}_{\text{avg}}(\cdot)$% in distribution (or on sample path) 
. However, %as one can imagine, 
it is extremely difficult to establish delay optimality or near delay optimality results when the job sizes are arbitrarily given. 
By using work-efficiency ordering, we obtain the following sufficient condition for near delay optimality in minimizing ${D}_{\text{avg}}(\cdot)$ for general job sizes.

%In Sec. \ref{sec_analysis}, we will use this sufficient condition to study near delay-optimal scheduling of task replications for arbitrary job sizes.  


\begin{theorem}\label{lem1}
If there exists a work-conserving policy $P\in\Pi$ such that for all $\mathcal{I}$
\begin{itemize}
\itemsep0em 
\item[1.] Policy $P$ is {more work-efficient} than any policy $\pi\in\Pi$,
\item[2.] In policy $P$, each task allocated to the servers belongs to the job with the fewest unassigned tasks, whenever there exist unassigned tasks in the queue,
\end{itemize} 
then \emph{$[{D}_{\text{avg}}(\bm{V}_{}(P))|\mathcal{I}]\leq_{\text{st}} [{D}_{\text{avg}}(\bm{C}_{}(\pi))|\mathcal{I}]$} holds for all $\pi\in\Pi$ and $\mathcal{I}$.
\end{theorem}

%The sufficient condition of Theorem \ref{lem1} provides a unified treatment for minimizing ${D}_{\text{avg}}(\cdot)$ in various system settings. 


We note that, in Theorem \ref{lem1} and other sufficient conditions of this section, model-specific information (such as the number of servers and service time distribution) and policy-specific information (such as when to replicate a task and replicate on which servers) is summarized in the work-efficiency ordering. 
%In Section \ref{sec_analysis} and Section \ref{sec_distributed}, 
When applying these sufficient conditions, one needs to first prove the work-efficiency ordering between policy $P$ and any policy $\pi\in\Pi$ for the specified system setting, and then uses these sufficient conditions to show that policy $P$ is near delay-optimal. 

%When using this sufficient condition i
%does not specify one particular queueing model or service time distribution, because such 

%This sufficient condition not depend on the specific queueing model or service time distribution. For each specific system setting, this  as long as a work-efficiency ordering can be established between 



The difficulties in proving Theorem \ref{lem1} are as follows: First, policy $P$ is a dynamic priority policy where the job with the fewest unassigned tasks has the highest priority. Hence, the priority of a job increases as more tasks of this job are assigned to the servers. On the other hand, policy $\pi$ could be any policy in $\Pi$, which may follow a  different priority rule. Therefore,  the servers might be processing completely different jobs in policy $P$ and policy $\pi$, which makes it difficult to compare these two policies. Second, policy $P$ is an online policy, where the scheduling decisions are made without using any information about the future job arrivals. However, policy $\pi$ is allowed to have access to the parameters $(a_i,{k}_i,d_i)$ of future arriving jobs. Hence, the comparison between these two policies is unfair for policy $P$. Third, all policies in $\Pi$ are non-preemptive and server-idleness is allowed for some policies in $\Pi$. These conditions are adversary for finding a delay-optimal or near-optimal policy in $\Pi$ \cite{michael2012book,Gittins:11}. 

%Even if Lemma \ref{thm1} switches to seek for near-delay optimality result, it is unclear 

%suggests that in such adverse scenarios, it is still possible to establish near-delay optimality results.  
%The difficulties in Theorem \ref{lem1} are as follows: 

%



%we consider preemption is not allowed and server-idleness is allowed for the policies in $\Pi$, which makes it extremely difficult to find a delay-optimal policy in $\Pi$ \cite{michael2012book,Gittins:11}. Lemma \ref{thm1} suggests that it is still possible to seek for near delay optimality in such adverse scenario.  of delay optimality, it is still possible to prove Lemma \ref{thm1}. 


%Second,  Second, while policy $P$ is an online policy, policy $\pi$ may have access to the parameters $(a_i,{k}_i,d_i)$ of future arriving jobs. Hence, the comparison between these two policies is unfair for policy $P$. Third, in $\Pi$ are , which is usually 

In order to prove Theorem \ref{lem1}, we need to first define the system state for any policy $\pi\in\Pi$. 

\begin{definition}\label{def_state_thm3}
At any time $t$, the system state of policy $\pi$ is specified by a pair of $n$-vectors $\bm{\xi}_{\pi}(t)=(\xi_{1,\pi}(t),\ldots,\xi_{n,\pi}(t))$ and $\bm{\gamma}_{\pi}(t)=(\gamma_{1,\pi}(t),\ldots,\gamma_{n,\pi}(t))$ %and $\bm{\zeta}=(\zeta_1,\ldots,\zeta_n)$ 
with non-negative components, where $n$ is the number of arriving jobs which can be either finite or infinite. The components of $\bm{\xi}_{\pi}(t)$ and $\bm{\gamma}_{\pi}(t)$ are interpreted as follows:
if job $i$ is present in the system at time $t$, then $\xi_{i,\pi}(t)$ is the number of remaining tasks (which are stored in the queue or being executed  by the servers) of job $i$, and $\gamma_{i,\pi}(t)$ is the number of unassigned tasks (which are stored in the queue and not being executed  by the servers) of job $i$; if job $i$ is not present in the system at time $t$ (i.e., job $i$ has not arrived at the system or has departed from the system), then $\xi_{i,\pi}(t)=\gamma_{i,\pi}(t)=0$. Hence, for all $i=1,\ldots,n$, $\pi\in\Pi$, and $t\in[0,\infty)$
\begin{align}%\label{eq_def_state_thm3}
0\leq \gamma_{i,\pi}(t)\leq \xi_{i,\pi}(t)\leq k_i.
\end{align}
Let $\{\bm{\xi}_{\pi}(t),\bm{\gamma}_{\pi}(t),t\geq0\}$ be the state process of policy $\pi$, which is assumed to be right-continuous. 
\end{definition}





A proof sketch of Theorem \ref{lem1} is provided as follows.
\begin{proof}[Proof sketch of Theorem \ref{lem1}]
%Here is a proof sketch of Theorem \ref{lem1}.
The proof contains two parts: In the first part, we use the conditions of Theorem \ref{lem1} to establish the following stochastic ordering result:
\begin{lemma}[Stochastic Ordering]\label{lemG4}
Suppose that $\bm{\xi}_{P}(0^-) = \bm{\gamma}_{P}(0^-) =\bm{\xi}_{\pi}(0^-) = \bm{\gamma}_{\pi}(0^-)=\bm{0}$ and the conditions of Theorem \ref{lem1} are satisfied. Then, the following relationship holds in stochastic ordering:
\begin{eqnarray}\label{eq_lemG4}
\sum_{i=j}^n {\gamma}_{[i],P}(t)\leq \sum_{i=j}^n {\xi}_{[i],\pi}(t),~j = 1,2,\ldots,n
\end{eqnarray}
for all $t\geq0$, where ${\xi}_{[i],\pi}(t)$ is the $i$-th largest component of vector $\bm{\xi}_{\pi}(t)$, and ${\gamma}_{[i],\pi}(t)$ is the $i$-th largest component of vector $\bm{\gamma}_{\pi}(t)$. 
\end{lemma}
From the perspective of majorization, \eqref{eq_lemG4} can be equivalent expressed as: $\bm{\xi}_{\pi}(t)$ is weakly majorized by $\bm{\gamma}_{P}(t)$ from above, i.e., $\bm{\xi}_{\pi}(t)\prec^{\text{w}}\bm{\gamma}_{P}(t)$ \cite{Marshall2011}. Note that Lemma \ref{lemG4} is a strong statement, because it holds for all $j = 1,2,\ldots,n$, time $t\in[0,\infty)$, job parameters $\mathcal{I}$, and policy $\pi\in\Pi$. In addition, Lemma \ref{lemG4} holds even if  the scheduling decisions of policy $\pi$ are made by using the parameters $(a_i,{k}_i,d_i)$ of future arriving jobs. In the second part of the proof, we use Lemma \ref{lemG4} to show that 
\begin{align}\label{eq_sketch1}
v_{(i)}(P) \leq c_{(i)}(\pi), ~i=1,\ldots,n
\end{align}
holds in stochastic ordering (Lemma \ref{lem_sample_path_ordering}).\footnote{Recall that $c_{(i)}(\pi)$ is the $i$-th smallest job completion time on the sample path of policy $\pi$, $v_{(i)}(P)$ is the $i$-th smallest component of the vector $(v_1(P),\ldots,v_n(P))$, and  $v_{i}(P)$ is the earliest time that all tasks of job $i$ are either completed or under service on the sample path of policy $P$.} Hence, Lemma \ref{lemG4} characterizes the timeline of job
executions on the sample paths of policy $P$ and policy $\pi$. Finally, Theorem \ref{lem1} follows from \eqref{eq_sketch1}. 
The proof details are provided in Appendix \ref{app0}. 
\end{proof}

%In Appendix \ref{app0}, we develop a  {sample-path ordering} technique to prove Theorem \ref{lem1}. 

%The first part of this {sample-path ordering} technique, i.e., 
The stochastic ordering result in Lemma \ref{lemG4} is motivated by \cite{Smith78}, which provided a proof of the optimality of Shortest-Remaining-Processing-Time (SRPT) first policy for single-server queueing systems. The generalization from \cite{Smith78} to Lemma \ref{lemG4} for multiple-server queueing systems with parallel processing and task replications is highly non-trivial. A preliminary version of this {sample-path ordering} technique was proposed in \cite{Sun2015}.  


%Nonetheless, this technique is able to establish a dominance between $v_{(i)}(P)$ and $c_{(i)}(\pi)$ on sample-path, hence the name. 




% but the generalization from \cite{Smith78} to this {sample-path ordering} technique is non-trivial. % and unexpected when this research started. 


%While existing delay optimality analyses of task replications \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013,ShengboInfocom,Sun2015} focused on the average delay ${D}_{\text{avg}}(\cdot)$, 
First, Theorem \ref{lem1} can be generalized to all delay metrics in $\mathcal{D}_{\text{sym}}$.
\begin{corollary}\label{coro1}
If \emph{${D}_{\text{avg}}(\cdot)$} is replaced by any \emph{$f\in\mathcal{D}_{\text{sym}}$}, Theorem \ref{lem1} still holds.
\end{corollary}

\begin{proof}
See Appendix \ref{app0}.
\end{proof}

\ifreport
\else
Due to space limitation, the proofs of the remaining results are relegated to our technical report \cite{report2015}.
\fi
In addition, a sufficient condition can be obtained for near optimality in minimizing the maximum lateness $L_{\max}(\cdot)$.
\begin{theorem}\label{lem2}
If there exists a work-conserving policy $P\in\Pi$ such that for all $\mathcal{I}$
\begin{itemize}
\itemsep0em 
\item[1.] Policy $P$ is {more work-efficient} than any policy $\pi\in\Pi$,
\item[2.] In policy $P$, each task allocated to the servers belongs to the job  with the earliest due time, whenever there exist unassigned tasks in the queue,
\end{itemize} 
then \emph{$[L_{\max}(\bm{V}_{}(P))|\mathcal{I}]\leq_{\text{st}} [L_{\max}(\bm{C}_{}(\pi))|\mathcal{I}]$} holds for all $\pi\in\Pi$ and $\mathcal{I}$.
\end{theorem}
%For the ease of understanding, Theorem \ref{lem1} and Theorem \ref{lem2} are expressed in similar forms. However, some parts of their proofs are quite different. In particular, because the delay metric is changed from average delay ${D}_{\text{avg}}(\cdot)$ to maximum lateness $L_{\max}(\cdot)$, a different form of sample-path ordering is required to prove Theorem \ref{lem2}. 
\ifreport
\begin{proof}[Proof sketch of Theorem \ref{lem2}]
The proof contains two parts: In the first part, we use the conditions of Theorem \ref{lem2} to establish a second form of  stochastic ordering:

\begin{lemma}[Stochastic Ordering --- The Second Form]\label{lemG4_thm3}
Suppose that $\bm{\xi}_P(0^-)=\bm{\gamma}_P(0^-)=\bm{\xi}_{\pi}(0^-)=\bm{\gamma}_{\pi}(0^-)=\bm{0}$ and the conditions of Thoerem \ref{lem2} are satisfied. Then, the following relationship holds in stochastic ordering:
\begin{eqnarray}\label{eq_lemG4_thm3}
\sum_{i:d_i\leq\tau} \gamma_{i,P}(t)\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}(t), ~\forall~\tau\in[0,\infty)
\end{eqnarray}
holds for all $t\geq0$.
\end{lemma}
In the second part of the proof, we use Lemma \ref{lemG4_thm3} to show that 
\begin{align}
v_{i}(P)-d_i \leq \max_{j=1,\ldots,n}[c_{j}(\pi)-d_j],~i=1,\ldots,n
\end{align}
holds in stochastic ordering (Lemma \ref{lem_sample_path_ordering_thm3}). By this, Theorem \ref{lem2} follows. The details are provided in Appendix \ref{app0_1}.
\end{proof}
\fi




If each job has one task, Theorem \ref{lem2} can be generalized to all delay metrics in $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$ by using the rearrangement inequality in \cite[Theorem 6.F.14]{Marshall2011} and\cite{Chang93rearrangement_majorization}. 
%This result is motivated by .
%, but the proof technique is different.
\begin{corollary}\label{coro2}
If $k_1=\ldots=k_n=1$ and \emph{$L_{\max}(\cdot)$} is replaced by any \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$}, Theorem \ref{lem2} still holds.
\end{corollary}
\ifreport
\begin{proof}[Proof sketch of Corollary \ref{coro2}]
For all $f\in\mathcal{D}_{\text{sym}}$, we use Corollary \ref{coro1} to prove that the statement of Theorem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$. For all $f\in\mathcal{D}_{\text{Sch-1}}$, we show that there exists an $n$-vector $\bm{u}'$ satisfying 
%In order to prove \eqref{eq_coro2_3}, 
%it is sufficient to show that there exists an  such that 
\begin{align}\label{eq_coro2_6}
\bm{u}(P)-\bm{d}\prec \bm{u}'- \bm{d} \leq \bm{c} (\pi)-\bm{d},
\end{align}
which further implies 
\begin{align}\label{eq_coro2_3}
\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}. 
\end{align} 
Using this, we can show that the statement of Theorem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{Sch-1}}$.
The details are provided Appendix \ref{app0_1}.
\end{proof}
\fi

If $d_i=a_i$ for all job $i$, $L_{\max}(\cdot)$ reduces to the {maximum delay} $D_{\max}(\cdot)$. In this case, we can obtain
\begin{theorem}\label{lem3}
If there exists a work-conserving policy $P\in\Pi$ such that for all $\mathcal{I}$
\begin{itemize}
\itemsep0em 
\item[1.] Policy $P$ is {more work-efficient} than any policy $\pi\in\Pi$,
\item[2.] In policy $P$, each task allocated to the servers belongs to the job  with the earliest arrival time, whenever there exist unassigned tasks in the queue,
\end{itemize} 
then \emph{$[D_{\max}(\bm{V}_{}(P))|\mathcal{I}]\leq_{\text{st}} [D_{\max}(\bm{C}_{}(\pi))|\mathcal{I}]$} holds for all $\pi\in\Pi$ and $\mathcal{I}$.
\end{theorem}
\ifreport
\begin{proof}
%Because $D_{\max}(\cdot)$ is a special case of $L_{\max}(\cdot)$. 
See Appendix \ref{app0_2}.
\end{proof}
\fi

If each job has $k$ tasks, Theorem \ref{lem3} can be generalized to all delay metrics in $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$.
\begin{corollary}\label{coro3_1}
If $k_1=\ldots=k_n=k$ and \emph{$D_{\max}(\cdot)$} is replaced by any \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$}, Theorem \ref{lem3} still holds.
\end{corollary}
\ifreport
\begin{proof}
See Appendix \ref{app0_2}.
\end{proof}
\fi

